Evidence for modification of $b$ quark hadronization in high-multiplicity $pp$ collisions at $\sqrt{s} = 13$ TeV

The production rate of $B^{0}_{s}$ mesons relative to $B^{0}$ mesons is measured by the LHCb experiment in $pp$ collisions at a center-of-mass energy $\sqrt{s} = 13$ TeV over the forward rapidity interval $2<y<4.5$ as a function of the charged particle multiplicity measured in the event. Evidence at the 3.4$\sigma$ level is found for an increase of the ratio of $B^{0}_{s}$ to $B^{0}$ cross-sections with multiplicity at transverse momenta below 6 GeV/$c$, with no significant multiplicity dependence at higher transverse momentum. Comparison with data from $e^{+}e^{-}$ collisions implies that the density of the hadronic medium may affect the production rates of $B$ mesons. This is qualitatively consistent with the emergence of quark coalescence as an additional hadronization mechanism in high-multiplicity collisions.

==> Authorship_LHCb-PAPER-2022-001.tex <==
% LHCb collaboration author list
% Data extracted on June 23rd, 2023 at 9:44pm for paper reference LHCb-PAPER-2022-001
\centerline
{\large\bf LHCb collaboration}
\begin
{flushleft}
\small
R.~Aaij$^{32}$\lhcborcid{0000-0003-0533-1952},
A.S.W.~Abdelmotteleb$^{50}$\lhcborcid{0000-0001-7905-0542},
C.~Abellan~Beteta$^{44}$,
F.~Abudin{\'e}n$^{50}$\lhcborcid{0000-0002-6737-3528},
T.~Ackernley$^{54}$\lhcborcid{0000-0002-5951-3498},
B.~Adeva$^{40}$\lhcborcid{0000-0001-9756-3712},
M.~Adinolfi$^{48}$\lhcborcid{0000-0002-1326-1264},
H.~Afsharnia$^{9}$,
C.~Agapopoulou$^{13}$\lhcborcid{0000-0002-2368-0147},
C.A.~Aidala$^{76}$\lhcborcid{0000-0001-9540-4988},
S.~Aiola$^{25}$\lhcborcid{0000-0001-6209-7627},
Z.~Ajaltouni$^{9}$,
S.~Akar$^{59}$\lhcborcid{0000-0003-0288-9694},
K.~Akiba$^{32}$\lhcborcid{0000-0002-6736-471X},
J.~Albrecht$^{15}$\lhcborcid{0000-0001-8636-1621},
F.~Alessio$^{42}$\lhcborcid{0000-0001-5317-1098},
M.~Alexander$^{53}$\lhcborcid{0000-0002-8148-2392},
A.~Alfonso~Albero$^{39}$\lhcborcid{0000-0001-6025-0675},
Z.~Aliouche$^{56}$\lhcborcid{0000-0003-0897-4160},
P.~Alvarez~Cartelle$^{49}$\lhcborcid{0000-0003-1652-2834},
S.~Amato$^{2}$\lhcborcid{0000-0002-3277-0662},
J.L.~Amey$^{48}$\lhcborcid{0000-0002-2597-3808},
Y.~Amhis$^{11,42}$\lhcborcid{0000-0003-4282-1512},
L.~An$^{42}$\lhcborcid{0000-0002-3274-5627},
L.~Anderlini$^{22}$\lhcborcid{0000-0001-6808-2418},
M.~Andersson$^{44}$\lhcborcid{0000-0003-3594-9163},
A.~Andreianov$^{38}$\lhcborcid{0000-0002-6273-0506},
M.~Andreotti$^{21}$\lhcborcid{0000-0003-2918-1311},
D.~Andreou$^{62}$\lhcborcid{0000-0001-6288-0558},
D.~Ao$^{6}$\lhcborcid{0000-0003-1647-4238},
F.~Archilli$^{17}$\lhcborcid{0000-0002-1779-6813},
A.~Artamonov$^{38}$\lhcborcid{0000-0002-2785-2233},
M.~Artuso$^{62}$\lhcborcid{0000-0002-5991-7273},
E.~Aslanides$^{10}$\lhcborcid{0000-0003-3286-683X},
M.~Atzeni$^{44}$\lhcborcid{0000-0002-3208-3336},
B.~Audurier$^{12}$\lhcborcid{0000-0001-9090-4254},
S.~Bachmann$^{17}$\lhcborcid{0000-0002-1186-3894},
M.~Bachmayer$^{43}$\lhcborcid{0000-0001-5996-2747},
J.J.~Back$^{50}$\lhcborcid{0000-0001-7791-4490},
A.~Bailly-reyre$^{13}$,
P.~Baladron~Rodriguez$^{40}$\lhcborcid{0000-0003-4240-2094},
V.~Balagura$^{12}$\lhcborcid{0000-0002-1611-7188},
W.~Baldini$^{21}$\lhcborcid{0000-0001-7658-8777},
J.~Baptista~de~Souza~Leite$^{1}$\lhcborcid{0000-0002-4442-5372},
M.~Barbetti$^{22,j}$\lhcborcid{0000-0002-6704-6914},
R.J.~Barlow$^{56}$\lhcborcid{0000-0002-8295-8612},
S.~Barsuk$^{11}$\lhcborcid{0000-0002-0898-6551},
W.~Barter$^{55}$\lhcborcid{0000-0002-9264-4799},
M.~Bartolini$^{49}$\lhcborcid{0000-0002-8479-5802},
F.~Baryshnikov$^{38}$\lhcborcid{0000-0002-6418-6428},
J.M.~Basels$^{14}$\lhcborcid{0000-0001-5860-8770},
G.~Bassi$^{29,p}$\lhcborcid{0000-0002-2145-3805},
B.~Batsukh$^{4}$\lhcborcid{0000-0003-1020-2549},
A.~Battig$^{15}$\lhcborcid{0009-0001-6252-960X},
A.~Bay$^{43}$\lhcborcid{0000-0002-4862-9399},
A.~Beck$^{50}$\lhcborcid{0000-0003-4872-1213},
M.~Becker$^{15}$\lhcborcid{0000-0002-7972-8760},
F.~Bedeschi$^{29}$\lhcborcid{0000-0002-8315-2119},
I.B.~Bediaga$^{1}$\lhcborcid{0000-0001-7806-5283},
A.~Beiter$^{62}$,
V.~Belavin$^{38}$,
S.~Belin$^{40}$\lhcborcid{0000-0001-7154-1304},
V.~Bellee$^{44}$\lhcborcid{0000-0001-5314-0953},
K.~Belous$^{38}$\lhcborcid{0000-0003-0014-2589},
I.~Belov$^{38}$\lhcborcid{0000-0003-1699-9202},
I.~Belyaev$^{38}$\lhcborcid{0000-0002-7458-7030},
G.~Bencivenni$^{23}$\lhcborcid{0000-0002-5107-0610},
E.~Ben-Haim$^{13}$\lhcborcid{0000-0002-9510-8414},
A.~Berezhnoy$^{38}$\lhcborcid{0000-0002-4431-7582},
R.~Bernet$^{44}$\lhcborcid{0000-0002-4856-8063},
D.~Berninghoff$^{17}$,
H.C.~Bernstein$^{62}$,
C.~Bertella$^{56}$\lhcborcid{0000-0002-3160-147X},
A.~Bertolin$^{28}$\lhcborcid{0000-0003-1393-4315},
C.~Betancourt$^{44}$\lhcborcid{0000-0001-9886-7427},
F.~Betti$^{42}$\lhcborcid{0000-0002-2395-235X},
Ia.~Bezshyiko$^{44}$\lhcborcid{0000-0002-4315-6414},
S.~Bhasin$^{48}$\lhcborcid{0000-0002-0146-0717},
J.~Bhom$^{35}$\lhcborcid{0000-0002-9709-903X},
L.~Bian$^{67}$\lhcborcid{0000-0001-5209-5097},
M.S.~Bieker$^{15}$\lhcborcid{0000-0001-7113-7862},
N.V.~Biesuz$^{21}$\lhcborcid{0000-0003-3004-0946},
S.~Bifani$^{47}$\lhcborcid{0000-0001-7072-4854},
P.~Billoir$^{13}$\lhcborcid{0000-0001-5433-9876},
A.~Biolchini$^{32}$\lhcborcid{0000-0001-6064-9993},
M.~Birch$^{55}$\lhcborcid{0000-0001-9157-4461},
F.C.R.~Bishop$^{49}$\lhcborcid{0000-0002-0023-3897},
A.~Bitadze$^{56}$\lhcborcid{0000-0001-7979-1092},
A.~Bizzeti$^{}$\lhcborcid{0000-0001-5729-5530},
M.~Bj{\o}rn$^{57}$,
M.P.~Blago$^{49}$\lhcborcid{0000-0001-7542-2388},
T.~Blake$^{50}$\lhcborcid{0000-0002-0259-5891},
F.~Blanc$^{43}$\lhcborcid{0000-0001-5775-3132},
S.~Blusk$^{62}$\lhcborcid{0000-0001-9170-684X},
D.~Bobulska$^{53}$\lhcborcid{0000-0002-3003-9980},
J.A.~Boelhauve$^{15}$\lhcborcid{0000-0002-3543-9959},
O.~Boente~Garcia$^{40}$\lhcborcid{0000-0003-0261-8085},
T.~Boettcher$^{59}$\lhcborcid{0000-0002-2439-9955},
A.~Boldyrev$^{38}$\lhcborcid{0000-0002-7872-6819},
N.~Bondar$^{38,42}$\lhcborcid{0000-0003-2714-9879},
S.~Borghi$^{56}$\lhcborcid{0000-0001-5135-1511},
M.~Borsato$^{17}$\lhcborcid{0000-0001-5760-2924},
J.T.~Borsuk$^{35}$\lhcborcid{0000-0002-9065-9030},
S.A.~Bouchiba$^{43}$\lhcborcid{0000-0002-0044-6470},
T.J.V.~Bowcock$^{54,42}$\lhcborcid{0000-0002-3505-6915},
A.~Boyer$^{42}$\lhcborcid{0000-0002-9909-0186},
C.~Bozzi$^{21}$\lhcborcid{0000-0001-6782-3982},
M.J.~Bradley$^{55}$,
S.~Braun$^{60}$\lhcborcid{0000-0002-4489-1314},
A.~Brea~Rodriguez$^{40}$\lhcborcid{0000-0001-5650-445X},
J.~Brodzicka$^{35}$\lhcborcid{0000-0002-8556-0597},
A.~Brossa~Gonzalo$^{50}$\lhcborcid{0000-0002-4442-1048},
D.~Brundu$^{27}$\lhcborcid{0000-0003-4457-5896},
A.~Buonaura$^{44}$\lhcborcid{0000-0003-4907-6463},
L.~Buonincontri$^{28}$\lhcborcid{0000-0002-1480-454X},
A.T.~Burke$^{56}$\lhcborcid{0000-0003-0243-0517},
C.~Burr$^{42}$\lhcborcid{0000-0002-5155-1094},
A.~Bursche$^{66}$,
A.~Butkevich$^{38}$\lhcborcid{0000-0001-9542-1411},
J.S.~Butter$^{32}$\lhcborcid{0000-0002-1816-536X},
J.~Buytaert$^{42}$\lhcborcid{0000-0002-7958-6790},
W.~Byczynski$^{42}$\lhcborcid{0009-0008-0187-3395},
S.~Cadeddu$^{27}$\lhcborcid{0000-0002-7763-500X},
H.~Cai$^{67}$,
R.~Calabrese$^{21,i}$\lhcborcid{0000-0002-1354-5400},
L.~Calefice$^{15,13}$\lhcborcid{0000-0001-6401-1583},
S.~Cali$^{23}$\lhcborcid{0000-0001-9056-0711},
R.~Calladine$^{47}$,
M.~Calvi$^{26,m}$\lhcborcid{0000-0002-8797-1357},
M.~Calvo~Gomez$^{74}$\lhcborcid{0000-0001-5588-1448},
P.~Camargo~Magalhaes$^{48}$\lhcborcid{0000-0003-3641-8110},
P.~Campana$^{23}$\lhcborcid{0000-0001-8233-1951},
D.H.~Campora~Perez$^{73}$\lhcborcid{0000-0001-8998-9975},
A.F.~Campoverde~Quezada$^{6}$\lhcborcid{0000-0003-1968-1216},
S.~Capelli$^{26,m}$\lhcborcid{0000-0002-8444-4498},
L.~Capriotti$^{20,g}$\lhcborcid{0000-0003-4899-0587},
A.~Carbone$^{20,g}$\lhcborcid{0000-0002-7045-2243},
G.~Carboni$^{31}$\lhcborcid{0000-0003-1128-8276},
R.~Cardinale$^{24,k}$\lhcborcid{0000-0002-7835-7638},
A.~Cardini$^{27}$\lhcborcid{0000-0002-6649-0298},
I.~Carli$^{4}$\lhcborcid{0000-0002-0411-1141},
P.~Carniti$^{26,m}$\lhcborcid{0000-0002-7820-2732},
L.~Carus$^{14}$,
A.~Casais~Vidal$^{40}$\lhcborcid{0000-0003-0469-2588},
R.~Caspary$^{17}$\lhcborcid{0000-0002-1449-1619},
G.~Casse$^{54}$\lhcborcid{0000-0002-8516-237X},
M.~Cattaneo$^{42}$\lhcborcid{0000-0001-7707-169X},
G.~Cavallero$^{42}$\lhcborcid{0000-0002-8342-7047},
V.~Cavallini$^{21,i}$\lhcborcid{0000-0001-7601-129X},
S.~Celani$^{43}$\lhcborcid{0000-0003-4715-7622},
J.~Cerasoli$^{10}$\lhcborcid{0000-0001-9777-881X},
D.~Cervenkov$^{57}$\lhcborcid{0000-0002-1865-741X},
A.J.~Chadwick$^{54}$\lhcborcid{0000-0003-3537-9404},
M.G.~Chapman$^{48}$,
M.~Charles$^{13}$\lhcborcid{0000-0003-4795-498X},
Ph.~Charpentier$^{42}$\lhcborcid{0000-0001-9295-8635},
C.A.~Chavez~Barajas$^{54}$\lhcborcid{0000-0002-4602-8661},
M.~Chefdeville$^{8}$\lhcborcid{0000-0002-6553-6493},
C.~Chen$^{3}$\lhcborcid{0000-0002-3400-5489},
S.~Chen$^{4}$\lhcborcid{0000-0002-8647-1828},
A.~Chernov$^{35}$\lhcborcid{0000-0003-0232-6808},
S.~Chernyshenko$^{46}$\lhcborcid{0000-0002-2546-6080},
V.~Chobanova$^{40}$\lhcborcid{0000-0002-1353-6002},
S.~Cholak$^{43}$\lhcborcid{0000-0001-8091-4766},
M.~Chrzaszcz$^{35}$\lhcborcid{0000-0001-7901-8710},
A.~Chubykin$^{38}$\lhcborcid{0000-0003-1061-9643},
V.~Chulikov$^{38}$\lhcborcid{0000-0002-7767-9117},
P.~Ciambrone$^{23}$\lhcborcid{0000-0003-0253-9846},
M.F.~Cicala$^{50}$\lhcborcid{0000-0003-0678-5809},
X.~Cid~Vidal$^{40}$\lhcborcid{0000-0002-0468-541X},
G.~Ciezarek$^{42}$\lhcborcid{0000-0003-1002-8368},
G.~Ciullo$^{i,21}$\lhcborcid{0000-0001-8297-2206},
P.E.L.~Clarke$^{52}$\lhcborcid{0000-0003-3746-0732},
M.~Clemencic$^{42}$\lhcborcid{0000-0003-1710-6824},
H.V.~Cliff$^{49}$\lhcborcid{0000-0003-0531-0916},
J.~Closier$^{42}$\lhcborcid{0000-0002-0228-9130},
J.L.~Cobbledick$^{56}$\lhcborcid{0000-0002-5146-9605},
V.~Coco$^{42}$\lhcborcid{0000-0002-5310-6808},
J.A.B.~Coelho$^{11}$\lhcborcid{0000-0001-5615-3899},
J.~Cogan$^{10}$\lhcborcid{0000-0001-7194-7566},
E.~Cogneras$^{9}$\lhcborcid{0000-0002-8933-9427},
L.~Cojocariu$^{37}$\lhcborcid{0000-0002-1281-5923},
P.~Collins$^{42}$\lhcborcid{0000-0003-1437-4022},
T.~Colombo$^{42}$\lhcborcid{0000-0002-9617-9687},
L.~Congedo$^{19,f}$\lhcborcid{0000-0003-4536-4644},
A.~Contu$^{27}$\lhcborcid{0000-0002-3545-2969},
N.~Cooke$^{47}$\lhcborcid{0000-0002-4179-3700},
G.~Coombs$^{53}$\lhcborcid{0000-0003-4621-2757},
I.~Corredoira~$^{40}$\lhcborcid{0000-0002-6089-0899},
G.~Corti$^{42}$\lhcborcid{0000-0003-2857-4471},
B.~Couturier$^{42}$\lhcborcid{0000-0001-6749-1033},
D.C.~Craik$^{58}$\lhcborcid{0000-0002-3684-1560},
J.~Crkovsk\'{a}$^{61}$\lhcborcid{0000-0002-7946-7580},
M.~Cruz~Torres$^{1,e}$\lhcborcid{0000-0003-2607-131X},
R.~Currie$^{52}$\lhcborcid{0000-0002-0166-9529},
C.L.~Da~Silva$^{61}$\lhcborcid{0000-0003-4106-8258},
S.~Dadabaev$^{38}$\lhcborcid{0000-0002-0093-3244},
L.~Dai$^{65}$\lhcborcid{0000-0002-4070-4729},
E.~Dall'Occo$^{15}$\lhcborcid{0000-0001-9313-4021},
J.~Dalseno$^{40}$\lhcborcid{0000-0003-3288-4683},
C.~D'Ambrosio$^{42}$\lhcborcid{0000-0003-4344-9994},
A.~Danilina$^{38}$\lhcborcid{0000-0003-3121-2164},
P.~d'Argent$^{15}$\lhcborcid{0000-0003-2380-8355},
J.E.~Davies$^{56}$\lhcborcid{0000-0002-5382-8683},
A.~Davis$^{56}$\lhcborcid{0000-0001-9458-5115},
O.~De~Aguiar~Francisco$^{56}$\lhcborcid{0000-0003-2735-678X},
J.~de~Boer$^{42}$\lhcborcid{0000-0002-6084-4294},
K.~De~Bruyn$^{72}$\lhcborcid{0000-0002-0615-4399},
S.~De~Capua$^{56}$\lhcborcid{0000-0002-6285-9596},
M.~De~Cian$^{43}$\lhcborcid{0000-0002-1268-9621},
U.~De~Freitas~Carneiro~Da~Graca$^{1}$\lhcborcid{0000-0003-0451-4028},
E.~De~Lucia$^{23}$\lhcborcid{0000-0003-0793-0844},
J.M.~De~Miranda$^{1}$\lhcborcid{0009-0003-2505-7337},
L.~De~Paula$^{2}$\lhcborcid{0000-0002-4984-7734},
M.~De~Serio$^{19,f}$\lhcborcid{0000-0003-4915-7933},
D.~De~Simone$^{44}$\lhcborcid{0000-0001-8180-4366},
P.~De~Simone$^{23}$\lhcborcid{0000-0001-9392-2079},
F.~De~Vellis$^{15}$\lhcborcid{0000-0001-7596-5091},
J.A.~de~Vries$^{73}$\lhcborcid{0000-0003-4712-9816},
C.T.~Dean$^{61}$\lhcborcid{0000-0002-6002-5870},
F.~Debernardis$^{19,f}$\lhcborcid{0009-0001-5383-4899},
D.~Decamp$^{8}$\lhcborcid{0000-0001-9643-6762},
V.~Dedu$^{10}$\lhcborcid{0000-0001-5672-8672},
L.~Del~Buono$^{13}$\lhcborcid{0000-0003-4774-2194},
B.~Delaney$^{49}$\lhcborcid{0009-0007-6371-8035},
H.-P.~Dembinski$^{15}$\lhcborcid{0000-0003-3337-3850},
V.~Denysenko$^{44}$\lhcborcid{0000-0002-0455-5404},
O.~Deschamps$^{9}$\lhcborcid{0000-0002-7047-6042},
F.~Dettori$^{27,h}$\lhcborcid{0000-0003-0256-8663},
B.~Dey$^{70}$\lhcborcid{0000-0002-4563-5806},
A.~Di~Cicco$^{23}$\lhcborcid{0000-0002-6925-8056},
P.~Di~Nezza$^{23}$\lhcborcid{0000-0003-4894-6762},
S.~Didenko$^{38}$\lhcborcid{0000-0001-5671-5863},
L.~Dieste~Maronas$^{40}$,
S.~Ding$^{62}$\lhcborcid{0000-0002-5946-581X},
V.~Dobishuk$^{46}$\lhcborcid{0000-0001-9004-3255},
A.~Dolmatov$^{38}$,
C.~Dong$^{3}$\lhcborcid{0000-0003-3259-6323},
A.M.~Donohoe$^{18}$\lhcborcid{0000-0002-4438-3950},
F.~Dordei$^{27}$\lhcborcid{0000-0002-2571-5067},
A.C.~dos~Reis$^{1}$\lhcborcid{0000-0001-7517-8418},
L.~Douglas$^{53}$,
A.G.~Downes$^{8}$\lhcborcid{0000-0003-0217-762X},
M.W.~Dudek$^{35}$\lhcborcid{0000-0003-3939-3262},
L.~Dufour$^{42}$\lhcborcid{0000-0002-3924-2774},
V.~Duk$^{71}$\lhcborcid{0000-0001-6440-0087},
P.~Durante$^{42}$\lhcborcid{0000-0002-1204-2270},
J.M.~Durham$^{61}$\lhcborcid{0000-0002-5831-3398},
D.~Dutta$^{56}$\lhcborcid{0000-0002-1191-3978},
A.~Dziurda$^{35}$\lhcborcid{0000-0003-4338-7156},
A.~Dzyuba$^{38}$\lhcborcid{0000-0003-3612-3195},
S.~Easo$^{51}$\lhcborcid{0000-0002-4027-7333},
U.~Egede$^{63}$\lhcborcid{0000-0001-5493-0762},
V.~Egorychev$^{38}$\lhcborcid{0000-0002-2539-673X},
S.~Eidelman$^{38,\dagger}$,
S.~Eisenhardt$^{52}$\lhcborcid{0000-0002-4860-6779},
S.~Ek-In$^{43}$\lhcborcid{0000-0002-2232-6760},
L.~Eklund$^{75}$\lhcborcid{0000-0002-2014-3864},
S.~Ely$^{62}$\lhcborcid{0000-0003-1618-3617},
A.~Ene$^{37}$\lhcborcid{0000-0001-5513-0927},
E.~Epple$^{61}$\lhcborcid{0000-0002-6312-3740},
S.~Escher$^{14}$\lhcborcid{0009-0007-2540-4203},
J.~Eschle$^{44}$\lhcborcid{0000-0002-7312-3699},
S.~Esen$^{44}$\lhcborcid{0000-0003-2437-8078},
T.~Evans$^{56}$\lhcborcid{0000-0003-3016-1879},
L.N.~Falcao$^{1}$\lhcborcid{0000-0003-3441-583X},
Y.~Fan$^{6}$\lhcborcid{0000-0002-3153-430X},
B.~Fang$^{67}$\lhcborcid{0000-0003-0030-3813},
S.~Farry$^{54}$\lhcborcid{0000-0001-5119-9740},
D.~Fazzini$^{26,m}$\lhcborcid{0000-0002-5938-4286},
M.~Feo$^{42}$\lhcborcid{0000-0001-5266-2442},
A.D.~Fernez$^{60}$\lhcborcid{0000-0001-9900-6514},
F.~Ferrari$^{20}$\lhcborcid{0000-0002-3721-4585},
L.~Ferreira~Lopes$^{43}$\lhcborcid{0009-0003-5290-823X},
F.~Ferreira~Rodrigues$^{2}$\lhcborcid{0000-0002-4274-5583},
S.~Ferreres~Sole$^{32}$\lhcborcid{0000-0003-3571-7741},
M.~Ferrillo$^{44}$\lhcborcid{0000-0003-1052-2198},
M.~Ferro-Luzzi$^{42}$\lhcborcid{0009-0008-1868-2165},
S.~Filippov$^{38}$\lhcborcid{0000-0003-3900-3914},
R.A.~Fini$^{19}$\lhcborcid{0000-0002-3821-3998},
M.~Fiorini$^{21,i}$\lhcborcid{0000-0001-6559-2084},
M.~Firlej$^{34}$\lhcborcid{0000-0002-1084-0084},
K.M.~Fischer$^{57}$\lhcborcid{0009-0000-8700-9910},
D.S.~Fitzgerald$^{76}$\lhcborcid{0000-0001-6862-6876},
C.~Fitzpatrick$^{56}$\lhcborcid{0000-0003-3674-0812},
T.~Fiutowski$^{34}$\lhcborcid{0000-0003-2342-8854},
F.~Fleuret$^{12}$\lhcborcid{0000-0002-2430-782X},
M.~Fontana$^{13}$\lhcborcid{0000-0003-4727-831X},
F.~Fontanelli$^{24,k}$\lhcborcid{0000-0001-7029-7178},
R.~Forty$^{42}$\lhcborcid{0000-0003-2103-7577},
D.~Foulds-Holt$^{49}$\lhcborcid{0000-0001-9921-687X},
V.~Franco~Lima$^{54}$\lhcborcid{0000-0002-3761-209X},
M.~Franco~Sevilla$^{60}$\lhcborcid{0000-0002-5250-2948},
M.~Frank$^{42}$\lhcborcid{0000-0002-4625-559X},
E.~Franzoso$^{21,i}$\lhcborcid{0000-0003-2130-1593},
G.~Frau$^{17}$\lhcborcid{0000-0003-3160-482X},
C.~Frei$^{42}$\lhcborcid{0000-0001-5501-5611},
D.A.~Friday$^{53}$\lhcborcid{0000-0001-9400-3322},
J.~Fu$^{6}$\lhcborcid{0000-0003-3177-2700},
Q.~Fuehring$^{15}$\lhcborcid{0000-0003-3179-2525},
E.~Gabriel$^{32}$\lhcborcid{0000-0001-8300-5939},
G.~Galati$^{19,f}$\lhcborcid{0000-0001-7348-3312},
A.~Gallas~Torreira$^{40}$\lhcborcid{0000-0002-2745-7954},
D.~Galli$^{20,g}$\lhcborcid{0000-0003-2375-6030},
S.~Gambetta$^{52,42}$\lhcborcid{0000-0003-2420-0501},
Y.~Gan$^{3}$\lhcborcid{0009-0006-6576-9293},
M.~Gandelman$^{2}$\lhcborcid{0000-0001-8192-8377},
P.~Gandini$^{25}$\lhcborcid{0000-0001-7267-6008},
Y.~Gao$^{5}$\lhcborcid{0000-0003-1484-0943},
M.~Garau$^{27,h}$\lhcborcid{0000-0002-0505-9584},
L.M.~Garcia~Martin$^{50}$\lhcborcid{0000-0003-0714-8991},
P.~Garcia~Moreno$^{39}$\lhcborcid{0000-0002-3612-1651},
J.~Garc{\'\i}a~Pardi{\~n}as$^{26,m}$\lhcborcid{0000-0003-2316-8829},
B.~Garcia~Plana$^{40}$,
F.A.~Garcia~Rosales$^{12}$\lhcborcid{0000-0003-4395-0244},
L.~Garrido$^{39}$\lhcborcid{0000-0001-8883-6539},
C.~Gaspar$^{42}$\lhcborcid{0000-0002-8009-1509},
R.E.~Geertsema$^{32}$\lhcborcid{0000-0001-6829-7777},
D.~Gerick$^{17}$,
L.L.~Gerken$^{15}$\lhcborcid{0000-0002-6769-3679},
E.~Gersabeck$^{56}$\lhcborcid{0000-0002-2860-6528},
M.~Gersabeck$^{56}$\lhcborcid{0000-0002-0075-8669},
T.~Gershon$^{50}$\lhcborcid{0000-0002-3183-5065},
L.~Giambastiani$^{28}$\lhcborcid{0000-0002-5170-0635},
V.~Gibson$^{49}$\lhcborcid{0000-0002-6661-1192},
H.K.~Giemza$^{36}$\lhcborcid{0000-0003-2597-8796},
A.L.~Gilman$^{57}$\lhcborcid{0000-0001-5934-7541},
M.~Giovannetti$^{23,s}$\lhcborcid{0000-0003-2135-9568},
A.~Giovent{\`u}$^{40}$\lhcborcid{0000-0001-5399-326X},
P.~Gironella~Gironell$^{39}$\lhcborcid{0000-0001-5603-4750},
C.~Giugliano$^{21,i}$\lhcborcid{0000-0002-6159-4557},
K.~Gizdov$^{52}$\lhcborcid{0000-0002-3543-7451},
E.L.~Gkougkousis$^{42}$\lhcborcid{0000-0002-2132-2071},
V.V.~Gligorov$^{13,42}$\lhcborcid{0000-0002-8189-8267},
C.~G{\"o}bel$^{64}$\lhcborcid{0000-0003-0523-495X},
E.~Golobardes$^{74}$\lhcborcid{0000-0001-8080-0769},
D.~Golubkov$^{38}$\lhcborcid{0000-0001-6216-1596},
A.~Golutvin$^{55,38}$\lhcborcid{0000-0003-2500-8247},
A.~Gomes$^{1,2,a,\dagger}$\lhcborcid{0009-0005-2892-2968},
S.~Gomez~Fernandez$^{39}$\lhcborcid{0000-0002-3064-9834},
F.~Goncalves~Abrantes$^{57}$\lhcborcid{0000-0002-7318-482X},
M.~Goncerz$^{35}$\lhcborcid{0000-0002-9224-914X},
G.~Gong$^{3}$\lhcborcid{0000-0002-7822-3947},
I.V.~Gorelov$^{38}$\lhcborcid{0000-0001-5570-0133},
C.~Gotti$^{26}$\lhcborcid{0000-0003-2501-9608},
J.P.~Grabowski$^{17}$\lhcborcid{0000-0001-8461-8382},
T.~Grammatico$^{13}$\lhcborcid{0000-0002-2818-9744},
L.A.~Granado~Cardoso$^{42}$\lhcborcid{0000-0003-2868-2173},
E.~Graug{\'e}s$^{39}$\lhcborcid{0000-0001-6571-4096},
E.~Graverini$^{43}$\lhcborcid{0000-0003-4647-6429},
G.~Graziani$^{}$\lhcborcid{0000-0001-8212-846X},
A. T.~Grecu$^{37}$\lhcborcid{0000-0002-7770-1839},
L.M.~Greeven$^{32}$\lhcborcid{0000-0001-5813-7972},
N.A.~Grieser$^{4}$\lhcborcid{0000-0003-0386-4923},
L.~Grillo$^{53}$\lhcborcid{0000-0001-5360-0091},
S.~Gromov$^{38}$\lhcborcid{0000-0002-8967-3644},
B.R.~Gruberg~Cazon$^{57}$\lhcborcid{0000-0003-4313-3121},
C. ~Gu$^{3}$\lhcborcid{0000-0001-5635-6063},
M.~Guarise$^{21,i}$\lhcborcid{0000-0001-8829-9681},
M.~Guittiere$^{11}$\lhcborcid{0000-0002-2916-7184},
P. A.~G{\"u}nther$^{17}$\lhcborcid{0000-0002-4057-4274},
E.~Gushchin$^{38}$\lhcborcid{0000-0001-8857-1665},
A.~Guth$^{14}$,
Y.~Guz$^{38}$\lhcborcid{0000-0001-7552-400X},
T.~Gys$^{42}$\lhcborcid{0000-0002-6825-6497},
T.~Hadavizadeh$^{63}$\lhcborcid{0000-0001-5730-8434},
G.~Haefeli$^{43}$\lhcborcid{0000-0002-9257-839X},
C.~Haen$^{42}$\lhcborcid{0000-0002-4947-2928},
J.~Haimberger$^{42}$\lhcborcid{0000-0002-3363-7783},
S.C.~Haines$^{49}$\lhcborcid{0000-0001-5906-391X},
T.~Halewood-leagas$^{54}$\lhcborcid{0000-0001-9629-7029},
M.M.~Halvorsen$^{42}$\lhcborcid{0000-0003-0959-3853},
P.M.~Hamilton$^{60}$\lhcborcid{0000-0002-2231-1374},
J.~Hammerich$^{54}$\lhcborcid{0000-0002-5556-1775},
Q.~Han$^{7}$\lhcborcid{0000-0002-7958-2917},
X.~Han$^{17}$\lhcborcid{0000-0001-7641-7505},
E.B.~Hansen$^{56}$\lhcborcid{0000-0002-5019-1648},
S.~Hansmann-Menzemer$^{17,42}$\lhcborcid{0000-0002-3804-8734},
L.~Hao$^{6}$\lhcborcid{0000-0001-8162-4277},
N.~Harnew$^{57}$\lhcborcid{0000-0001-9616-6651},
T.~Harrison$^{54}$\lhcborcid{0000-0002-1576-9205},
C.~Hasse$^{42}$\lhcborcid{0000-0002-9658-8827},
M.~Hatch$^{42}$\lhcborcid{0009-0004-4850-7465},
J.~He$^{6,c}$\lhcborcid{0000-0002-1465-0077},
K.~Heijhoff$^{32}$\lhcborcid{0000-0001-5407-7466},
K.~Heinicke$^{15}$\lhcborcid{0009-0003-8781-3425},
R.D.L.~Henderson$^{63,50}$\lhcborcid{0000-0001-6445-4907},
A.M.~Hennequin$^{58}$\lhcborcid{0009-0008-7974-3785},
K.~Hennessy$^{54}$\lhcborcid{0000-0002-1529-8087},
L.~Henry$^{42}$\lhcborcid{0000-0003-3605-832X},
J.~Heuel$^{14}$\lhcborcid{0000-0001-9384-6926},
A.~Hicheur$^{2}$\lhcborcid{0000-0002-3712-7318},
D.~Hill$^{43}$\lhcborcid{0000-0003-2613-7315},
M.~Hilton$^{56}$\lhcborcid{0000-0001-7703-7424},
S.E.~Hollitt$^{15}$\lhcborcid{0000-0002-4962-3546},
R.~Hou$^{7}$\lhcborcid{0000-0002-3139-3332},
Y.~Hou$^{8}$\lhcborcid{0000-0001-6454-278X},
J.~Hu$^{17}$,
J.~Hu$^{66}$\lhcborcid{0000-0002-8227-4544},
W.~Hu$^{7}$\lhcborcid{0000-0002-2855-0544},
X.~Hu$^{3}$\lhcborcid{0000-0002-5924-2683},
W.~Huang$^{6}$\lhcborcid{0000-0002-1407-1729},
X.~Huang$^{67}$,
W.~Hulsbergen$^{32}$\lhcborcid{0000-0003-3018-5707},
R.J.~Hunter$^{50}$\lhcborcid{0000-0001-7894-8799},
M.~Hushchyn$^{38}$\lhcborcid{0000-0002-8894-6292},
D.~Hutchcroft$^{54}$\lhcborcid{0000-0002-4174-6509},
P.~Ibis$^{15}$\lhcborcid{0000-0002-2022-6862},
M.~Idzik$^{34}$\lhcborcid{0000-0001-6349-0033},
D.~Ilin$^{38}$\lhcborcid{0000-0001-8771-3115},
P.~Ilten$^{59}$\lhcborcid{0000-0001-5534-1732},
A.~Inglessi$^{38}$\lhcborcid{0000-0002-2522-6722},
A.~Iniukhin$^{38}$\lhcborcid{0000-0002-1940-6276},
A.~Ishteev$^{38}$\lhcborcid{0000-0003-1409-1428},
K.~Ivshin$^{38}$\lhcborcid{0000-0001-8403-0706},
R.~Jacobsson$^{42}$\lhcborcid{0000-0003-4971-7160},
H.~Jage$^{14}$\lhcborcid{0000-0002-8096-3792},
S.~Jakobsen$^{42}$\lhcborcid{0000-0002-6564-040X},
E.~Jans$^{32}$\lhcborcid{0000-0002-5438-9176},
B.K.~Jashal$^{41}$\lhcborcid{0000-0002-0025-4663},
A.~Jawahery$^{60}$\lhcborcid{0000-0003-3719-119X},
V.~Jevtic$^{15}$\lhcborcid{0000-0001-6427-4746},
X.~Jiang$^{4,6}$\lhcborcid{0000-0001-8120-3296},
M.~John$^{57}$\lhcborcid{0000-0002-8579-844X},
D.~Johnson$^{58}$\lhcborcid{0000-0003-3272-6001},
C.R.~Jones$^{49}$\lhcborcid{0000-0003-1699-8816},
T.P.~Jones$^{50}$\lhcborcid{0000-0001-5706-7255},
B.~Jost$^{42}$\lhcborcid{0009-0005-4053-1222},
N.~Jurik$^{42}$\lhcborcid{0000-0002-6066-7232},
S.~Kandybei$^{45}$\lhcborcid{0000-0003-3598-0427},
Y.~Kang$^{3}$\lhcborcid{0000-0002-6528-8178},
M.~Karacson$^{42}$\lhcborcid{0009-0006-1867-9674},
D.~Karpenkov$^{38}$\lhcborcid{0000-0001-8686-2303},
M.~Karpov$^{38}$\lhcborcid{0000-0003-4503-2682},
J.W.~Kautz$^{59}$\lhcborcid{0000-0001-8482-5576},
F.~Keizer$^{42}$\lhcborcid{0000-0002-1290-6737},
D.M.~Keller$^{62}$\lhcborcid{0000-0002-2608-1270},
M.~Kenzie$^{50}$\lhcborcid{0000-0001-7910-4109},
T.~Ketel$^{33}$\lhcborcid{0000-0002-9652-1964},
B.~Khanji$^{15}$\lhcborcid{0000-0003-3838-281X},
A.~Kharisova$^{38}$\lhcborcid{0000-0002-5291-9583},
S.~Kholodenko$^{38}$\lhcborcid{0000-0002-0260-6570},
T.~Kirn$^{14}$\lhcborcid{0000-0002-0253-8619},
V.S.~Kirsebom$^{43}$\lhcborcid{0009-0005-4421-9025},
O.~Kitouni$^{58}$\lhcborcid{0000-0001-9695-8165},
S.~Klaver$^{33}$\lhcborcid{0000-0001-7909-1272},
N.~Kleijne$^{29,p}$\lhcborcid{0000-0003-0828-0943},
K.~Klimaszewski$^{36}$\lhcborcid{0000-0003-0741-5922},
M.R.~Kmiec$^{36}$\lhcborcid{0000-0002-1821-1848},
S.~Koliiev$^{46}$\lhcborcid{0009-0002-3680-1224},
A.~Kondybayeva$^{38}$\lhcborcid{0000-0001-8727-6840},
A.~Konoplyannikov$^{38}$\lhcborcid{0009-0005-2645-8364},
P.~Kopciewicz$^{34}$\lhcborcid{0000-0001-9092-3527},
R.~Kopecna$^{17}$,
P.~Koppenburg$^{32}$\lhcborcid{0000-0001-8614-7203},
M.~Korolev$^{38}$\lhcborcid{0000-0002-7473-2031},
I.~Kostiuk$^{32,46}$\lhcborcid{0000-0002-8767-7289},
O.~Kot$^{46}$,
S.~Kotriakhova$^{}$\lhcborcid{0000-0002-1495-0053},
A.~Kozachuk$^{38}$\lhcborcid{0000-0001-6805-0395},
P.~Kravchenko$^{38}$\lhcborcid{0000-0002-4036-2060},
L.~Kravchuk$^{38}$\lhcborcid{0000-0001-8631-4200},
R.D.~Krawczyk$^{42}$\lhcborcid{0000-0001-8664-4787},
M.~Kreps$^{50}$\lhcborcid{0000-0002-6133-486X},
S.~Kretzschmar$^{14}$\lhcborcid{0009-0008-8631-9552},
P.~Krokovny$^{38}$\lhcborcid{0000-0002-1236-4667},
W.~Krupa$^{34}$\lhcborcid{0000-0002-7947-465X},
W.~Krzemien$^{36}$\lhcborcid{0000-0002-9546-358X},
J.~Kubat$^{17}$,
W.~Kucewicz$^{35,34}$\lhcborcid{0000-0002-2073-711X},
M.~Kucharczyk$^{35}$\lhcborcid{0000-0003-4688-0050},
V.~Kudryavtsev$^{38}$\lhcborcid{0009-0000-2192-995X},
H.S.~Kuindersma$^{32}$,
G.J.~Kunde$^{61}$,
D.~Lacarrere$^{42}$\lhcborcid{0009-0005-6974-140X},
G.~Lafferty$^{56}$\lhcborcid{0000-0003-0658-4919},
A.~Lai$^{27}$\lhcborcid{0000-0003-1633-0496},
A.~Lampis$^{27,h}$\lhcborcid{0000-0002-5443-4870},
D.~Lancierini$^{44}$\lhcborcid{0000-0003-1587-4555},
J.J.~Lane$^{56}$\lhcborcid{0000-0002-5816-9488},
R.~Lane$^{48}$\lhcborcid{0000-0002-2360-2392},
G.~Lanfranchi$^{23}$\lhcborcid{0000-0002-9467-8001},
C.~Langenbruch$^{14}$\lhcborcid{0000-0002-3454-7261},
J.~Langer$^{15}$\lhcborcid{0000-0002-0322-5550},
O.~Lantwin$^{38}$\lhcborcid{0000-0003-2384-5973},
T.~Latham$^{50}$\lhcborcid{0000-0002-7195-8537},
F.~Lazzari$^{29,t}$\lhcborcid{0000-0002-3151-3453},
M.~Lazzaroni$^{25,l}$\lhcborcid{0000-0002-4094-1273},
R.~Le~Gac$^{10}$\lhcborcid{0000-0002-7551-6971},
S.H.~Lee$^{76}$\lhcborcid{0000-0003-3523-9479},
R.~Lef{\`e}vre$^{9}$\lhcborcid{0000-0002-6917-6210},
A.~Leflat$^{38}$\lhcborcid{0000-0001-9619-6666},
S.~Legotin$^{38}$\lhcborcid{0000-0003-3192-6175},
P.~Lenisa$^{i,21}$\lhcborcid{0000-0003-3509-1240},
O.~Leroy$^{10}$\lhcborcid{0000-0002-2589-240X},
T.~Lesiak$^{35}$\lhcborcid{0000-0002-3966-2998},
B.~Leverington$^{17}$\lhcborcid{0000-0001-6640-7274},
H.~Li$^{66}$\lhcborcid{0000-0002-2366-9554},
K.~Li$^{7}$\lhcborcid{0000-0002-2243-8412},
P.~Li$^{17}$\lhcborcid{0000-0003-2740-9765},
S.~Li$^{7}$\lhcborcid{0000-0001-5455-3768},
Y.~Li$^{4}$\lhcborcid{0000-0003-2043-4669},
Z.~Li$^{62}$\lhcborcid{0000-0003-0755-8413},
X.~Liang$^{62}$\lhcborcid{0000-0002-5277-9103},
C.~Lin$^{6}$\lhcborcid{0000-0001-7587-3365},
T.~Lin$^{55}$\lhcborcid{0000-0001-6052-8243},
R.~Lindner$^{42}$\lhcborcid{0000-0002-5541-6500},
V.~Lisovskyi$^{15}$\lhcborcid{0000-0003-4451-214X},
R.~Litvinov$^{27,h}$\lhcborcid{0000-0002-4234-435X},
G.~Liu$^{66}$\lhcborcid{0000-0001-5961-6588},
H.~Liu$^{6}$\lhcborcid{0000-0001-6658-1993},
Q.~Liu$^{6}$\lhcborcid{0000-0003-4658-6361},
S.~Liu$^{4,6}$\lhcborcid{0000-0002-6919-227X},
A.~Lobo~Salvia$^{39}$\lhcborcid{0000-0002-2375-9509},
A.~Loi$^{27}$\lhcborcid{0000-0003-4176-1503},
R.~Lollini$^{71}$\lhcborcid{0000-0003-3898-7464},
J.~Lomba~Castro$^{40}$\lhcborcid{0000-0003-1874-8407},
I.~Longstaff$^{53}$,
J.H.~Lopes$^{2}$\lhcborcid{0000-0003-1168-9547},
S.~L{\'o}pez~Soli{\~n}o$^{40}$\lhcborcid{0000-0001-9892-5113},
G.H.~Lovell$^{49}$\lhcborcid{0000-0002-9433-054X},
Y.~Lu$^{4,b}$\lhcborcid{0000-0003-4416-6961},
C.~Lucarelli$^{22,j}$\lhcborcid{0000-0002-8196-1828},
D.~Lucchesi$^{28,n}$\lhcborcid{0000-0003-4937-7637},
S.~Luchuk$^{38}$\lhcborcid{0000-0002-3697-8129},
M.~Lucio~Martinez$^{32}$\lhcborcid{0000-0001-6823-2607},
V.~Lukashenko$^{32,46}$\lhcborcid{0000-0002-0630-5185},
Y.~Luo$^{3}$\lhcborcid{0009-0001-8755-2937},
A.~Lupato$^{56}$\lhcborcid{0000-0003-0312-3914},
E.~Luppi$^{21,i}$\lhcborcid{0000-0002-1072-5633},
A.~Lusiani$^{29,p}$\lhcborcid{0000-0002-6876-3288},
K.~Lynch$^{18}$\lhcborcid{0000-0002-7053-4951},
X.-R.~Lyu$^{6}$\lhcborcid{0000-0001-5689-9578},
L.~Ma$^{4}$\lhcborcid{0009-0004-5695-8274},
R.~Ma$^{6}$\lhcborcid{0000-0002-0152-2412},
S.~Maccolini$^{20}$\lhcborcid{0000-0002-9571-7535},
F.~Machefert$^{11}$\lhcborcid{0000-0002-4644-5916},
F.~Maciuc$^{37}$\lhcborcid{0000-0001-6651-9436},
V.~Macko$^{43}$\lhcborcid{0009-0003-8228-0404},
P.~Mackowiak$^{15}$\lhcborcid{0009-0007-6216-7155},
S.~Maddrell-Mander$^{48}$,
L.R.~Madhan~Mohan$^{48}$\lhcborcid{0000-0002-9390-8821},
A.~Maevskiy$^{38}$\lhcborcid{0000-0003-1652-8005},
D.~Maisuzenko$^{38}$\lhcborcid{0000-0001-5704-3499},
M.W.~Majewski$^{34}$,
J.J.~Malczewski$^{35}$\lhcborcid{0000-0003-2744-3656},
S.~Malde$^{57}$\lhcborcid{0000-0002-8179-0707},
B.~Malecki$^{35}$\lhcborcid{0000-0003-0062-1985},
A.~Malinin$^{38}$\lhcborcid{0000-0002-3731-9977},
T.~Maltsev$^{38}$\lhcborcid{0000-0002-2120-5633},
H.~Malygina$^{17}$\lhcborcid{0000-0002-1807-3430},
G.~Manca$^{27,h}$\lhcborcid{0000-0003-1960-4413},
G.~Mancinelli$^{10}$\lhcborcid{0000-0003-1144-3678},
D.~Manuzzi$^{20}$\lhcborcid{0000-0002-9915-6587},
C.A.~Manzari$^{44}$\lhcborcid{0000-0001-8114-3078},
D.~Marangotto$^{25,l}$\lhcborcid{0000-0001-9099-4878},
J.F.~Marchand$^{8}$\lhcborcid{0000-0002-4111-0797},
U.~Marconi$^{20}$\lhcborcid{0000-0002-5055-7224},
S.~Mariani$^{22,j}$\lhcborcid{0000-0002-7298-3101},
C.~Marin~Benito$^{42}$\lhcborcid{0000-0003-0529-6982},
M.~Marinangeli$^{43}$\lhcborcid{0000-0002-8361-9356},
J.~Marks$^{17}$\lhcborcid{0000-0002-2867-722X},
A.M.~Marshall$^{48}$\lhcborcid{0000-0002-9863-4954},
P.J.~Marshall$^{54}$,
G.~Martelli$^{71,o}$\lhcborcid{0000-0002-6150-3168},
G.~Martellotti$^{30}$\lhcborcid{0000-0002-8663-9037},
L.~Martinazzoli$^{42,m}$\lhcborcid{0000-0002-8996-795X},
M.~Martinelli$^{26,m}$\lhcborcid{0000-0003-4792-9178},
D.~Martinez~Santos$^{40}$\lhcborcid{0000-0002-6438-4483},
F.~Martinez~Vidal$^{41}$\lhcborcid{0000-0001-6841-6035},
A.~Massafferri$^{1}$\lhcborcid{0000-0002-3264-3401},
M.~Materok$^{14}$\lhcborcid{0000-0002-7380-6190},
R.~Matev$^{42}$\lhcborcid{0000-0001-8713-6119},
A.~Mathad$^{44}$\lhcborcid{0000-0002-9428-4715},
V.~Matiunin$^{38}$\lhcborcid{0000-0003-4665-5451},
C.~Matteuzzi$^{26}$\lhcborcid{0000-0002-4047-4521},
K.R.~Mattioli$^{76}$\lhcborcid{0000-0003-2222-7727},
A.~Mauri$^{32}$\lhcborcid{0000-0003-1664-8963},
E.~Maurice$^{12}$\lhcborcid{0000-0002-7366-4364},
J.~Mauricio$^{39}$\lhcborcid{0000-0002-9331-1363},
M.~Mazurek$^{42}$\lhcborcid{0000-0002-3687-9630},
M.~McCann$^{55}$\lhcborcid{0000-0002-3038-7301},
L.~Mcconnell$^{18}$\lhcborcid{0009-0004-7045-2181},
T.H.~McGrath$^{56}$\lhcborcid{0000-0001-8993-3234},
N.T.~McHugh$^{53}$\lhcborcid{0000-0002-5477-3995},
A.~McNab$^{56}$\lhcborcid{0000-0001-5023-2086},
R.~McNulty$^{18}$\lhcborcid{0000-0001-7144-0175},
J.V.~Mead$^{54}$\lhcborcid{0000-0003-0875-2533},
B.~Meadows$^{59}$\lhcborcid{0000-0002-1947-8034},
G.~Meier$^{15}$\lhcborcid{0000-0002-4266-1726},
D.~Melnychuk$^{36}$\lhcborcid{0000-0003-1667-7115},
S.~Meloni$^{26,m}$\lhcborcid{0000-0003-1836-0189},
M.~Merk$^{32,73}$\lhcborcid{0000-0003-0818-4695},
A.~Merli$^{25,l}$\lhcborcid{0000-0002-0374-5310},
L.~Meyer~Garcia$^{2}$\lhcborcid{0000-0002-2622-8551},
M.~Mikhasenko$^{69,d}$\lhcborcid{0000-0002-6969-2063},
D.A.~Milanes$^{68}$\lhcborcid{0000-0001-7450-1121},
E.~Millard$^{50}$,
M.~Milovanovic$^{42}$\lhcborcid{0000-0003-1580-0898},
M.-N.~Minard$^{8,\dagger}$,
A.~Minotti$^{26,m}$\lhcborcid{0000-0002-0091-5177},
S.E.~Mitchell$^{52}$\lhcborcid{0000-0002-7956-054X},
B.~Mitreska$^{56}$\lhcborcid{0000-0002-1697-4999},
D.S.~Mitzel$^{15}$\lhcborcid{0000-0003-3650-2689},
A.~M{\"o}dden~$^{15}$\lhcborcid{0009-0009-9185-4901},
R.A.~Mohammed$^{57}$\lhcborcid{0000-0002-3718-4144},
R.D.~Moise$^{55}$\lhcborcid{0000-0002-5662-8804},
S.~Mokhnenko$^{38}$\lhcborcid{0000-0002-1849-1472},
T.~Momb{\"a}cher$^{40}$\lhcborcid{0000-0002-5612-979X},
I.A.~Monroy$^{68}$\lhcborcid{0000-0001-8742-0531},
S.~Monteil$^{9}$\lhcborcid{0000-0001-5015-3353},
M.~Morandin$^{28}$\lhcborcid{0000-0003-4708-4240},
G.~Morello$^{23}$\lhcborcid{0000-0002-6180-3697},
M.J.~Morello$^{29,p}$\lhcborcid{0000-0003-4190-1078},
J.~Moron$^{34}$\lhcborcid{0000-0002-1857-1675},
A.B.~Morris$^{69}$\lhcborcid{0000-0002-0832-9199},
A.G.~Morris$^{50}$\lhcborcid{0000-0001-6644-9888},
R.~Mountain$^{62}$\lhcborcid{0000-0003-1908-4219},
H.~Mu$^{3}$\lhcborcid{0000-0001-9720-7507},
F.~Muheim$^{52}$\lhcborcid{0000-0002-1131-8909},
M.~Mulder$^{72}$\lhcborcid{0000-0001-6867-8166},
K.~M{\"u}ller$^{44}$\lhcborcid{0000-0002-5105-1305},
C.H.~Murphy$^{57}$\lhcborcid{0000-0002-6441-075X},
D.~Murray$^{56}$\lhcborcid{0000-0002-5729-8675},
R.~Murta$^{55}$\lhcborcid{0000-0002-6915-8370},
P.~Muzzetto$^{27,h}$\lhcborcid{0000-0003-3109-3695},
P.~Naik$^{48}$\lhcborcid{0000-0001-6977-2971},
T.~Nakada$^{43}$\lhcborcid{0009-0000-6210-6861},
R.~Nandakumar$^{51}$\lhcborcid{0000-0002-6813-6794},
T.~Nanut$^{42}$\lhcborcid{0000-0002-5728-9867},
I.~Nasteva$^{2}$\lhcborcid{0000-0001-7115-7214},
M.~Needham$^{52}$\lhcborcid{0000-0002-8297-6714},
N.~Neri$^{25,l}$\lhcborcid{0000-0002-6106-3756},
S.~Neubert$^{69}$\lhcborcid{0000-0002-0706-1944},
N.~Neufeld$^{42}$\lhcborcid{0000-0003-2298-0102},
P.~Neustroev$^{38}$,
R.~Newcombe$^{55}$,
E.M.~Niel$^{43}$\lhcborcid{0000-0002-6587-4695},
S.~Nieswand$^{14}$,
N.~Nikitin$^{38}$\lhcborcid{0000-0003-0215-1091},
N.S.~Nolte$^{58}$\lhcborcid{0000-0003-2536-4209},
C.~Normand$^{8,h,27}$\lhcborcid{0000-0001-5055-7710},
C.~Nunez$^{76}$\lhcborcid{0000-0002-2521-9346},
A.~Oblakowska-Mucha$^{34}$\lhcborcid{0000-0003-1328-0534},
V.~Obraztsov$^{38}$\lhcborcid{0000-0002-0994-3641},
T.~Oeser$^{14}$\lhcborcid{0000-0001-7792-4082},
D.P.~O'Hanlon$^{48}$\lhcborcid{0000-0002-3001-6690},
S.~Okamura$^{21,i}$\lhcborcid{0000-0003-1229-3093},
R.~Oldeman$^{27,h}$\lhcborcid{0000-0001-6902-0710},
F.~Oliva$^{52}$\lhcborcid{0000-0001-7025-3407},
M.E.~Olivares$^{62}$,
C.J.G.~Onderwater$^{72}$\lhcborcid{0000-0002-2310-4166},
R.H.~O'Neil$^{52}$\lhcborcid{0000-0002-9797-8464},
J.M.~Otalora~Goicochea$^{2}$\lhcborcid{0000-0002-9584-8500},
T.~Ovsiannikova$^{38}$\lhcborcid{0000-0002-3890-9426},
P.~Owen$^{44}$\lhcborcid{0000-0002-4161-9147},
A.~Oyanguren$^{41}$\lhcborcid{0000-0002-8240-7300},
O.~Ozcelik$^{52}$\lhcborcid{0000-0003-3227-9248},
K.O.~Padeken$^{69}$\lhcborcid{0000-0001-7251-9125},
B.~Pagare$^{50}$\lhcborcid{0000-0003-3184-1622},
P.R.~Pais$^{42}$\lhcborcid{0009-0005-9758-742X},
T.~Pajero$^{57}$\lhcborcid{0000-0001-9630-2000},
A.~Palano$^{19}$\lhcborcid{0000-0002-6095-9593},
M.~Palutan$^{23}$\lhcborcid{0000-0001-7052-1360},
Y.~Pan$^{56}$\lhcborcid{0000-0002-4110-7299},
G.~Panshin$^{38}$\lhcborcid{0000-0001-9163-2051},
A.~Papanestis$^{51}$\lhcborcid{0000-0002-5405-2901},
M.~Pappagallo$^{19,f}$\lhcborcid{0000-0001-7601-5602},
L.L.~Pappalardo$^{21,i}$\lhcborcid{0000-0002-0876-3163},
C.~Pappenheimer$^{59}$\lhcborcid{0000-0003-0738-3668},
W.~Parker$^{60}$\lhcborcid{0000-0001-9479-1285},
C.~Parkes$^{56}$\lhcborcid{0000-0003-4174-1334},
B.~Passalacqua$^{21,i}$\lhcborcid{0000-0003-3643-7469},
G.~Passaleva$^{22}$\lhcborcid{0000-0002-8077-8378},
A.~Pastore$^{19}$\lhcborcid{0000-0002-5024-3495},
M.~Patel$^{55}$\lhcborcid{0000-0003-3871-5602},
C.~Patrignani$^{20,g}$\lhcborcid{0000-0002-5882-1747},
C.J.~Pawley$^{73}$\lhcborcid{0000-0001-9112-3724},
A.~Pearce$^{42}$\lhcborcid{0000-0002-9719-1522},
A.~Pellegrino$^{32}$\lhcborcid{0000-0002-7884-345X},
M.~Pepe~Altarelli$^{42}$\lhcborcid{0000-0002-1642-4030},
S.~Perazzini$^{20}$\lhcborcid{0000-0002-1862-7122},
D.~Pereima$^{38}$\lhcborcid{0000-0002-7008-8082},
A.~Pereiro~Castro$^{40}$\lhcborcid{0000-0001-9721-3325},
P.~Perret$^{9}$\lhcborcid{0000-0002-5732-4343},
M.~Petric$^{53}$,
K.~Petridis$^{48}$\lhcborcid{0000-0001-7871-5119},
A.~Petrolini$^{24,k}$\lhcborcid{0000-0003-0222-7594},
A.~Petrov$^{38}$,
S.~Petrucci$^{52}$\lhcborcid{0000-0001-8312-4268},
M.~Petruzzo$^{25}$\lhcborcid{0000-0001-8377-149X},
H.~Pham$^{62}$\lhcborcid{0000-0003-2995-1953},
A.~Philippov$^{38}$\lhcborcid{0000-0002-5103-8880},
R.~Piandani$^{6}$\lhcborcid{0000-0003-2226-8924},
L.~Pica$^{29,p}$\lhcborcid{0000-0001-9837-6556},
M.~Piccini$^{71}$\lhcborcid{0000-0001-8659-4409},
B.~Pietrzyk$^{8}$\lhcborcid{0000-0003-1836-7233},
G.~Pietrzyk$^{11}$\lhcborcid{0000-0001-9622-820X},
M.~Pili$^{57}$\lhcborcid{0000-0002-7599-4666},
D.~Pinci$^{30}$\lhcborcid{0000-0002-7224-9708},
F.~Pisani$^{42}$\lhcborcid{0000-0002-7763-252X},
M.~Pizzichemi$^{26,m,42}$\lhcborcid{0000-0001-5189-230X},
V.~Placinta$^{37}$\lhcborcid{0000-0003-4465-2441},
J.~Plews$^{47}$\lhcborcid{0009-0009-8213-7265},
M.~Plo~Casasus$^{40}$\lhcborcid{0000-0002-2289-918X},
F.~Polci$^{13,42}$\lhcborcid{0000-0001-8058-0436},
M.~Poli~Lener$^{23}$\lhcborcid{0000-0001-7867-1232},
M.~Poliakova$^{62}$,
A.~Poluektov$^{10}$\lhcborcid{0000-0003-2222-9925},
N.~Polukhina$^{38}$\lhcborcid{0000-0001-5942-1772},
I.~Polyakov$^{62}$\lhcborcid{0000-0002-6855-7783},
E.~Polycarpo$^{2}$\lhcborcid{0000-0002-4298-5309},
S.~Ponce$^{42}$\lhcborcid{0000-0002-1476-7056},
D.~Popov$^{6,42}$\lhcborcid{0000-0002-8293-2922},
S.~Popov$^{38}$\lhcborcid{0000-0003-2849-3233},
S.~Poslavskii$^{38}$\lhcborcid{0000-0003-3236-1452},
K.~Prasanth$^{35}$\lhcborcid{0000-0001-9923-0938},
L.~Promberger$^{42}$\lhcborcid{0000-0003-0127-6255},
C.~Prouve$^{40}$\lhcborcid{0000-0003-2000-6306},
V.~Pugatch$^{46}$\lhcborcid{0000-0002-5204-9821},
V.~Puill$^{11}$\lhcborcid{0000-0003-0806-7149},
G.~Punzi$^{29,q}$\lhcborcid{0000-0002-8346-9052},
H.R.~Qi$^{3}$\lhcborcid{0000-0002-9325-2308},
W.~Qian$^{6}$\lhcborcid{0000-0003-3932-7556},
N.~Qin$^{3}$\lhcborcid{0000-0001-8453-658X},
S.~Qu$^{3}$\lhcborcid{0000-0002-7518-0961},
R.~Quagliani$^{43}$\lhcborcid{0000-0002-3632-2453},
N.V.~Raab$^{18}$\lhcborcid{0000-0002-3199-2968},
R.I.~Rabadan~Trejo$^{6}$\lhcborcid{0000-0002-9787-3910},
B.~Rachwal$^{34}$\lhcborcid{0000-0002-0685-6497},
J.H.~Rademacker$^{48}$\lhcborcid{0000-0003-2599-7209},
R.~Rajagopalan$^{62}$,
M.~Rama$^{29}$\lhcborcid{0000-0003-3002-4719},
M.~Ramos~Pernas$^{50}$\lhcborcid{0000-0003-1600-9432},
M.S.~Rangel$^{2}$\lhcborcid{0000-0002-8690-5198},
F.~Ratnikov$^{38}$\lhcborcid{0000-0003-0762-5583},
G.~Raven$^{33,42}$\lhcborcid{0000-0002-2897-5323},
M.~Rebollo~De~Miguel$^{41}$\lhcborcid{0000-0002-4522-4863},
M.~Reboud$^{8}$\lhcborcid{0000-0001-6033-3606},
F.~Redi$^{42}$\lhcborcid{0000-0001-9728-8984},
F.~Reiss$^{56}$\lhcborcid{0000-0002-8395-7654},
C.~Remon~Alepuz$^{41}$,
Z.~Ren$^{3}$\lhcborcid{0000-0001-9974-9350},
V.~Renaudin$^{57}$\lhcborcid{0000-0003-4440-937X},
P.K.~Resmi$^{10}$\lhcborcid{0000-0001-9025-2225},
R.~Ribatti$^{29,p}$\lhcborcid{0000-0003-1778-1213},
A.M.~Ricci$^{27}$\lhcborcid{0000-0002-8816-3626},
S.~Ricciardi$^{51}$\lhcborcid{0000-0002-4254-3658},
K.~Rinnert$^{54}$\lhcborcid{0000-0001-9802-1122},
P.~Robbe$^{11}$\lhcborcid{0000-0002-0656-9033},
G.~Robertson$^{52}$\lhcborcid{0000-0002-7026-1383},
A.B.~Rodrigues$^{43}$\lhcborcid{0000-0002-1955-7541},
E.~Rodrigues$^{54}$\lhcborcid{0000-0003-2846-7625},
J.A.~Rodriguez~Lopez$^{68}$\lhcborcid{0000-0003-1895-9319},
E.~Rodriguez~Rodriguez$^{40}$\lhcborcid{0000-0002-7973-8061},
A.~Rollings$^{57}$\lhcborcid{0000-0002-5213-3783},
P.~Roloff$^{42}$\lhcborcid{0000-0001-7378-4350},
V.~Romanovskiy$^{38}$\lhcborcid{0000-0003-0939-4272},
M.~Romero~Lamas$^{40}$\lhcborcid{0000-0002-1217-8418},
A.~Romero~Vidal$^{40}$\lhcborcid{0000-0002-8830-1486},
J.D.~Roth$^{76,\dagger}$,
M.~Rotondo$^{23}$\lhcborcid{0000-0001-5704-6163},
M.S.~Rudolph$^{62}$\lhcborcid{0000-0002-0050-575X},
T.~Ruf$^{42}$\lhcborcid{0000-0002-8657-3576},
R.A.~Ruiz~Fernandez$^{40}$\lhcborcid{0000-0002-5727-4454},
J.~Ruiz~Vidal$^{41}$\lhcborcid{0000-0001-8362-7164},
A.~Ryzhikov$^{38}$\lhcborcid{0000-0002-3543-0313},
J.~Ryzka$^{34}$\lhcborcid{0000-0003-4235-2445},
J.J.~Saborido~Silva$^{40}$\lhcborcid{0000-0002-6270-130X},
N.~Sagidova$^{38}$\lhcborcid{0000-0002-2640-3794},
N.~Sahoo$^{47}$\lhcborcid{0000-0001-9539-8370},
B.~Saitta$^{27,h}$\lhcborcid{0000-0003-3491-0232},
M.~Salomoni$^{42}$\lhcborcid{0009-0007-9229-653X},
C.~Sanchez~Gras$^{32}$\lhcborcid{0000-0002-7082-887X},
I.~Sanderswood$^{41}$\lhcborcid{0000-0001-7731-6757},
R.~Santacesaria$^{30}$\lhcborcid{0000-0003-3826-0329},
C.~Santamarina~Rios$^{40}$\lhcborcid{0000-0002-9810-1816},
M.~Santimaria$^{23}$\lhcborcid{0000-0002-8776-6759},
E.~Santovetti$^{31,s}$\lhcborcid{0000-0002-5605-1662},
D.~Saranin$^{38}$\lhcborcid{0000-0002-9617-9986},
G.~Sarpis$^{14}$\lhcborcid{0000-0003-1711-2044},
M.~Sarpis$^{69}$\lhcborcid{0000-0002-6402-1674},
A.~Sarti$^{30}$\lhcborcid{0000-0001-5419-7951},
C.~Satriano$^{30,r}$\lhcborcid{0000-0002-4976-0460},
A.~Satta$^{31}$\lhcborcid{0000-0003-2462-913X},
M.~Saur$^{15}$\lhcborcid{0000-0001-8752-4293},
D.~Savrina$^{38}$\lhcborcid{0000-0001-8372-6031},
H.~Sazak$^{9}$\lhcborcid{0000-0003-2689-1123},
L.G.~Scantlebury~Smead$^{57}$\lhcborcid{0000-0001-8702-7991},
A.~Scarabotto$^{13}$\lhcborcid{0000-0003-2290-9672},
S.~Schael$^{14}$\lhcborcid{0000-0003-4013-3468},
S.~Scherl$^{54}$\lhcborcid{0000-0003-0528-2724},
M.~Schiller$^{53}$\lhcborcid{0000-0001-8750-863X},
H.~Schindler$^{42}$\lhcborcid{0000-0002-1468-0479},
M.~Schmelling$^{16}$\lhcborcid{0000-0003-3305-0576},
B.~Schmidt$^{42}$\lhcborcid{0000-0002-8400-1566},
S.~Schmitt$^{14}$\lhcborcid{0000-0002-6394-1081},
O.~Schneider$^{43}$\lhcborcid{0000-0002-6014-7552},
A.~Schopper$^{42}$\lhcborcid{0000-0002-8581-3312},
M.~Schubiger$^{32}$\lhcborcid{0000-0001-9330-1440},
S.~Schulte$^{43}$\lhcborcid{0009-0001-8533-0783},
M.H.~Schune$^{11}$\lhcborcid{0000-0002-3648-0830},
R.~Schwemmer$^{42}$\lhcborcid{0009-0005-5265-9792},
B.~Sciascia$^{23,42}$\lhcborcid{0000-0003-0670-006X},
A.~Sciuccati$^{42}$\lhcborcid{0000-0002-8568-1487},
S.~Sellam$^{40}$\lhcborcid{0000-0003-0383-1451},
A.~Semennikov$^{38}$\lhcborcid{0000-0003-1130-2197},
M.~Senghi~Soares$^{33}$\lhcborcid{0000-0001-9676-6059},
A.~Sergi$^{24,k}$\lhcborcid{0000-0001-9495-6115},
N.~Serra$^{44}$\lhcborcid{0000-0002-5033-0580},
L.~Sestini$^{28}$\lhcborcid{0000-0002-1127-5144},
A.~Seuthe$^{15}$\lhcborcid{0000-0002-0736-3061},
Y.~Shang$^{5}$\lhcborcid{0000-0001-7987-7558},
D.M.~Shangase$^{76}$\lhcborcid{0000-0002-0287-6124},
M.~Shapkin$^{38}$\lhcborcid{0000-0002-4098-9592},
I.~Shchemerov$^{38}$\lhcborcid{0000-0001-9193-8106},
L.~Shchutska$^{43}$\lhcborcid{0000-0003-0700-5448},
T.~Shears$^{54}$\lhcborcid{0000-0002-2653-1366},
L.~Shekhtman$^{38}$\lhcborcid{0000-0003-1512-9715},
Z.~Shen$^{5}$\lhcborcid{0000-0003-1391-5384},
S.~Sheng$^{4,6}$\lhcborcid{0000-0002-1050-5649},
V.~Shevchenko$^{38}$\lhcborcid{0000-0003-3171-9125},
E.B.~Shields$^{26,m}$\lhcborcid{0000-0001-5836-5211},
Y.~Shimizu$^{11}$\lhcborcid{0000-0002-4936-1152},
E.~Shmanin$^{38}$\lhcborcid{0000-0002-8868-1730},
J.D.~Shupperd$^{62}$\lhcborcid{0009-0006-8218-2566},
B.G.~Siddi$^{21,i}$\lhcborcid{0000-0002-3004-187X},
R.~Silva~Coutinho$^{44}$\lhcborcid{0000-0002-1545-959X},
G.~Simi$^{28}$\lhcborcid{0000-0001-6741-6199},
S.~Simone$^{19,f}$\lhcborcid{0000-0003-3631-8398},
M.~Singla$^{63}$\lhcborcid{0000-0003-3204-5847},
N.~Skidmore$^{56}$\lhcborcid{0000-0003-3410-0731},
R.~Skuza$^{17}$\lhcborcid{0000-0001-6057-6018},
T.~Skwarnicki$^{62}$\lhcborcid{0000-0002-9897-9506},
M.W.~Slater$^{47}$\lhcborcid{0000-0002-2687-1950},
I.~Slazyk$^{21,i}$\lhcborcid{0000-0002-3513-9737},
J.C.~Smallwood$^{57}$\lhcborcid{0000-0003-2460-3327},
J.G.~Smeaton$^{49}$\lhcborcid{0000-0002-8694-2853},
E.~Smith$^{44}$\lhcborcid{0000-0002-9740-0574},
M.~Smith$^{55}$\lhcborcid{0000-0002-3872-1917},
A.~Snoch$^{32}$\lhcborcid{0000-0001-6431-6360},
L.~Soares~Lavra$^{9}$\lhcborcid{0000-0002-2652-123X},
M.D.~Sokoloff$^{59}$\lhcborcid{0000-0001-6181-4583},
F.J.P.~Soler$^{53}$\lhcborcid{0000-0002-4893-3729},
A.~Solomin$^{38,48}$\lhcborcid{0000-0003-0644-3227},
A.~Solovev$^{38}$\lhcborcid{0000-0003-4254-6012},
I.~Solovyev$^{38}$\lhcborcid{0000-0003-4254-6012},
F.L.~Souza~De~Almeida$^{2}$\lhcborcid{0000-0001-7181-6785},
B.~Souza~De~Paula$^{2}$\lhcborcid{0009-0003-3794-3408},
B.~Spaan$^{15,\dagger}$,
E.~Spadaro~Norella$^{25,l}$\lhcborcid{0000-0002-1111-5597},
E.~Spiridenkov$^{38}$,
P.~Spradlin$^{53}$\lhcborcid{0000-0002-5280-9464},
V.~Sriskaran$^{42}$\lhcborcid{0000-0002-9867-0453},
F.~Stagni$^{42}$\lhcborcid{0000-0002-7576-4019},
M.~Stahl$^{59}$\lhcborcid{0000-0001-8476-8188},
S.~Stahl$^{42}$\lhcborcid{0000-0002-8243-400X},
S.~Stanislaus$^{57}$\lhcborcid{0000-0003-1776-0498},
O.~Steinkamp$^{44}$\lhcborcid{0000-0001-7055-6467},
O.~Stenyakin$^{38}$,
H.~Stevens$^{15}$\lhcborcid{0000-0002-9474-9332},
S.~Stone$^{62,\dagger}$\lhcborcid{0000-0002-2122-771X},
D.~Strekalina$^{38}$\lhcborcid{0000-0003-3830-4889},
F.~Suljik$^{57}$\lhcborcid{0000-0001-6767-7698},
J.~Sun$^{27}$\lhcborcid{0000-0002-6020-2304},
L.~Sun$^{67}$\lhcborcid{0000-0002-0034-2567},
Y.~Sun$^{60}$\lhcborcid{0000-0003-4933-5058},
P.~Svihra$^{56}$\lhcborcid{0000-0002-7811-2147},
P.N.~Swallow$^{47}$\lhcborcid{0000-0003-2751-8515},
K.~Swientek$^{34}$\lhcborcid{0000-0001-6086-4116},
A.~Szabelski$^{36}$\lhcborcid{0000-0002-6604-2938},
T.~Szumlak$^{34}$\lhcborcid{0000-0002-2562-7163},
M.~Szymanski$^{42}$\lhcborcid{0000-0002-9121-6629},
S.~Taneja$^{56}$\lhcborcid{0000-0001-8856-2777},
A.R.~Tanner$^{48}$,
M.D.~Tat$^{57}$\lhcborcid{0000-0002-6866-7085},
A.~Terentev$^{38}$\lhcborcid{0000-0003-2574-8560},
F.~Teubert$^{42}$\lhcborcid{0000-0003-3277-5268},
E.~Thomas$^{42}$\lhcborcid{0000-0003-0984-7593},
D.J.D.~Thompson$^{47}$\lhcborcid{0000-0003-1196-5943},
K.A.~Thomson$^{54}$\lhcborcid{0000-0003-3111-4003},
H.~Tilquin$^{55}$\lhcborcid{0000-0003-4735-2014},
V.~Tisserand$^{9}$\lhcborcid{0000-0003-4916-0446},
S.~T'Jampens$^{8}$\lhcborcid{0000-0003-4249-6641},
M.~Tobin$^{4}$\lhcborcid{0000-0002-2047-7020},
L.~Tomassetti$^{21,i}$\lhcborcid{0000-0003-4184-1335},
X.~Tong$^{5}$\lhcborcid{0000-0002-5278-1203},
D.~Torres~Machado$^{1}$\lhcborcid{0000-0001-7030-6468},
D.Y.~Tou$^{3}$\lhcborcid{0000-0002-4732-2408},
E.~Trifonova$^{38}$,
S.M.~Trilov$^{48}$\lhcborcid{0000-0003-0267-6402},
C.~Trippl$^{43}$\lhcborcid{0000-0003-3664-1240},
G.~Tuci$^{6}$\lhcborcid{0000-0002-0364-5758},
A.~Tully$^{43}$\lhcborcid{0000-0002-8712-9055},
N.~Tuning$^{32,42}$\lhcborcid{0000-0003-2611-7840},
A.~Ukleja$^{36}$\lhcborcid{0000-0003-0480-4850},
D.J.~Unverzagt$^{17}$\lhcborcid{0000-0002-1484-2546},
E.~Ursov$^{38}$\lhcborcid{0000-0002-6519-4526},
A.~Usachov$^{32}$\lhcborcid{0000-0002-5829-6284},
A.~Ustyuzhanin$^{38}$\lhcborcid{0000-0001-7865-2357},
U.~Uwer$^{17}$\lhcborcid{0000-0002-8514-3777},
A.~Vagner$^{38}$,
V.~Vagnoni$^{20}$\lhcborcid{0000-0003-2206-311X},
A.~Valassi$^{42}$\lhcborcid{0000-0001-9322-9565},
G.~Valenti$^{20}$\lhcborcid{0000-0002-6119-7535},
N.~Valls~Canudas$^{74}$\lhcborcid{0000-0001-8748-8448},
M.~van~Beuzekom$^{32}$\lhcborcid{0000-0002-0500-1286},
M.~Van~Dijk$^{43}$\lhcborcid{0000-0003-2538-5798},
H.~Van~Hecke$^{61}$\lhcborcid{0000-0001-7961-7190},
E.~van~Herwijnen$^{38}$\lhcborcid{0000-0001-8807-8811},
M.~van~Veghel$^{72}$\lhcborcid{0000-0001-6178-6623},
R.~Vazquez~Gomez$^{39}$\lhcborcid{0000-0001-5319-1128},
P.~Vazquez~Regueiro$^{40}$\lhcborcid{0000-0002-0767-9736},
C.~V{\'a}zquez~Sierra$^{42}$\lhcborcid{0000-0002-5865-0677},
S.~Vecchi$^{21}$\lhcborcid{0000-0002-4311-3166},
J.J.~Velthuis$^{48}$\lhcborcid{0000-0002-4649-3221},
M.~Veltri$^{22,u}$\lhcborcid{0000-0001-7917-9661},
A.~Venkateswaran$^{62}$\lhcborcid{0000-0001-6950-1477},
M.~Veronesi$^{32}$\lhcborcid{0000-0002-1916-3884},
M.~Vesterinen$^{50}$\lhcborcid{0000-0001-7717-2765},
D.~~Vieira$^{59}$\lhcborcid{0000-0001-9511-2846},
M.~Vieites~Diaz$^{43}$\lhcborcid{0000-0002-0944-4340},
X.~Vilasis-Cardona$^{74}$\lhcborcid{0000-0002-1915-9543},
E.~Vilella~Figueras$^{54}$\lhcborcid{0000-0002-7865-2856},
A.~Villa$^{20}$\lhcborcid{0000-0002-9392-6157},
P.~Vincent$^{13}$\lhcborcid{0000-0002-9283-4541},
F.C.~Volle$^{11}$\lhcborcid{0000-0003-1828-3881},
D.~vom~Bruch$^{10}$\lhcborcid{0000-0001-9905-8031},
A.~Vorobyev$^{38}$,
V.~Vorobyev$^{38}$,
N.~Voropaev$^{38}$\lhcborcid{0000-0002-2100-0726},
K.~Vos$^{73}$\lhcborcid{0000-0002-4258-4062},
R.~Waldi$^{17}$\lhcborcid{0000-0002-4778-3642},
J.~Walsh$^{29}$\lhcborcid{0000-0002-7235-6976},
C.~Wang$^{17}$\lhcborcid{0000-0002-5909-1379},
J.~Wang$^{5}$\lhcborcid{0000-0001-7542-3073},
J.~Wang$^{4}$\lhcborcid{0000-0002-6391-2205},
J.~Wang$^{3}$\lhcborcid{0000-0002-3281-8136},
J.~Wang$^{67}$\lhcborcid{0000-0001-6711-4465},
M.~Wang$^{5}$\lhcborcid{0000-0003-4062-710X},
R.~Wang$^{48}$\lhcborcid{0000-0002-2629-4735},
Y.~Wang$^{7}$\lhcborcid{0000-0003-3979-4330},
Z.~Wang$^{44}$\lhcborcid{0000-0002-5041-7651},
Z.~Wang$^{3}$\lhcborcid{0000-0003-0597-4878},
Z.~Wang$^{6}$\lhcborcid{0000-0003-4410-6889},
J.A.~Ward$^{50,63}$\lhcborcid{0000-0003-4160-9333},
N.K.~Watson$^{47}$\lhcborcid{0000-0002-8142-4678},
D.~Websdale$^{55}$\lhcborcid{0000-0002-4113-1539},
C.~Weisser$^{58}$,
B.D.C.~Westhenry$^{48}$\lhcborcid{0000-0002-4589-2626},
D.J.~White$^{56}$\lhcborcid{0000-0002-5121-6923},
M.~Whitehead$^{53}$\lhcborcid{0000-0002-2142-3673},
A.R.~Wiederhold$^{50}$\lhcborcid{0000-0002-1023-1086},
D.~Wiedner$^{15}$\lhcborcid{0000-0002-4149-4137},
G.~Wilkinson$^{57}$\lhcborcid{0000-0001-5255-0619},
M.K.~Wilkinson$^{59}$\lhcborcid{0000-0001-6561-2145},
I.~Williams$^{49}$,
M.~Williams$^{58}$\lhcborcid{0000-0001-8285-3346},
M.R.J.~Williams$^{52}$\lhcborcid{0000-0001-5448-4213},
F.F.~Wilson$^{51}$\lhcborcid{0000-0002-5552-0842},
W.~Wislicki$^{36}$\lhcborcid{0000-0001-5765-6308},
M.~Witek$^{35}$\lhcborcid{0000-0002-8317-385X},
L.~Witola$^{17}$\lhcborcid{0000-0001-9178-9921},
C.P.~Wong$^{61}$\lhcborcid{0000-0002-9839-4065},
G.~Wormser$^{11}$\lhcborcid{0000-0003-4077-6295},
S.A.~Wotton$^{49}$\lhcborcid{0000-0003-4543-8121},
H.~Wu$^{62}$\lhcborcid{0000-0002-9337-3476},
K.~Wyllie$^{42}$\lhcborcid{0000-0002-2699-2189},
Z.~Xiang$^{6}$\lhcborcid{0000-0002-9700-3448},
D.~Xiao$^{7}$\lhcborcid{0000-0003-4319-1305},
Y.~Xie$^{7}$\lhcborcid{0000-0001-5012-4069},
A.~Xu$^{5}$\lhcborcid{0000-0002-8521-1688},
J.~Xu$^{6}$\lhcborcid{0000-0001-6950-5865},
L.~Xu$^{3}$\lhcborcid{0000-0003-2800-1438},
M.~Xu$^{50}$\lhcborcid{0000-0001-8885-565X},
Q.~Xu$^{6}$,
Z.~Xu$^{9}$\lhcborcid{0000-0002-7531-6873},
Z.~Xu$^{6}$\lhcborcid{0000-0001-9558-1079},
D.~Yang$^{3}$\lhcborcid{0009-0002-2675-4022},
S.~Yang$^{6}$\lhcborcid{0000-0003-2505-0365},
Y.~Yang$^{6}$\lhcborcid{0000-0002-8917-2620},
Z.~Yang$^{5}$\lhcborcid{0000-0003-2937-9782},
Z.~Yang$^{60}$\lhcborcid{0000-0003-0572-2021},
Y.~Yao$^{62}$,
L.E.~Yeomans$^{54}$\lhcborcid{0000-0002-6737-0511},
H.~Yin$^{7}$\lhcborcid{0000-0001-6977-8257},
J.~Yu$^{65}$\lhcborcid{0000-0003-1230-3300},
X.~Yuan$^{62}$\lhcborcid{0000-0003-0468-3083},
E.~Zaffaroni$^{43}$\lhcborcid{0000-0003-1714-9218},
M.~Zavertyaev$^{16}$\lhcborcid{0000-0002-4655-715X},
M.~Zdybal$^{35}$\lhcborcid{0000-0002-1701-9619},
O.~Zenaiev$^{42}$\lhcborcid{0000-0003-3783-6330},
M.~Zeng$^{3}$\lhcborcid{0000-0001-9717-1751},
D.~Zhang$^{7}$\lhcborcid{0000-0002-8826-9113},
L.~Zhang$^{3}$\lhcborcid{0000-0003-2279-8837},
S.~Zhang$^{65}$\lhcborcid{0000-0002-9794-4088},
S.~Zhang$^{5}$\lhcborcid{0000-0002-2385-0767},
Y.~Zhang$^{5}$\lhcborcid{0000-0002-0157-188X},
Y.~Zhang$^{57}$,
A.~Zharkova$^{38}$\lhcborcid{0000-0003-1237-4491},
A.~Zhelezov$^{17}$\lhcborcid{0000-0002-2344-9412},
Y.~Zheng$^{6}$\lhcborcid{0000-0003-0322-9858},
T.~Zhou$^{5}$\lhcborcid{0000-0002-3804-9948},
X.~Zhou$^{6}$\lhcborcid{0009-0005-9485-9477},
Y.~Zhou$^{6}$\lhcborcid{0000-0003-2035-3391},
V.~Zhovkovska$^{11}$\lhcborcid{0000-0002-9812-4508},
X.~Zhu$^{3}$\lhcborcid{0000-0002-9573-4570},
X.~Zhu$^{7}$\lhcborcid{0000-0002-4485-1478},
Z.~Zhu$^{6}$\lhcborcid{0000-0002-9211-3867},
V.~Zhukov$^{14,38}$\lhcborcid{0000-0003-0159-291X},
Q.~Zou$^{4,6}$\lhcborcid{0000-0003-0038-5038},
S.~Zucchelli$^{20,g}$\lhcborcid{0000-0002-2411-1085},
D.~Zuliani$^{28}$\lhcborcid{0000-0002-1478-4593},
G.~Zunica$^{56}$\lhcborcid{0000-0002-5972-6290}.\bigskip

{\footnotesize \it

$^{1}$Centro Brasileiro de Pesquisas F{\'\i}sicas (CBPF), Rio de Janeiro, Brazil\\
$^{2}$Universidade Federal do Rio de Janeiro (UFRJ), Rio de Janeiro, Brazil\\
$^{3}$Center for High Energy Physics, Tsinghua University, Beijing, China\\
$^{4}$Institute Of High Energy Physics (IHEP), Beijing, China\\
$^{5}$School of Physics State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing, China\\
$^{6}$University of Chinese Academy of Sciences, Beijing, China\\
$^{7}$Institute of Particle Physics, Central China Normal University, Wuhan, Hubei, China\\
$^{8}$Universit{\'e} Savoie Mont Blanc, CNRS, IN2P3-LAPP, Annecy, France\\
$^{9}$Universit{\'e} Clermont Auvergne, CNRS/IN2P3, LPC, Clermont-Ferrand, France\\
$^{10}$Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France\\
$^{11}$Universit{\'e} Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France\\
$^{12}$Laboratoire Leprince-Ringuet, CNRS/IN2P3, Ecole Polytechnique, Institut Polytechnique de Paris, Palaiseau, France\\
$^{13}$LPNHE, Sorbonne Universit{\'e}, Paris Diderot Sorbonne Paris Cit{\'e}, CNRS/IN2P3, Paris, France\\
$^{14}$I. Physikalisches Institut, RWTH Aachen University, Aachen, Germany\\
$^{15}$Fakult{\"a}t Physik, Technische Universit{\"a}t Dortmund, Dortmund, Germany\\
$^{16}$Max-Planck-Institut f{\"u}r Kernphysik (MPIK), Heidelberg, Germany\\
$^{17}$Physikalisches Institut, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg, Germany\\
$^{18}$School of Physics, University College Dublin, Dublin, Ireland\\
$^{19}$INFN Sezione di Bari, Bari, Italy\\
$^{20}$INFN Sezione di Bologna, Bologna, Italy\\
$^{21}$INFN Sezione di Ferrara, Ferrara, Italy\\
$^{22}$INFN Sezione di Firenze, Firenze, Italy\\
$^{23}$INFN Laboratori Nazionali di Frascati, Frascati, Italy\\
$^{24}$INFN Sezione di Genova, Genova, Italy\\
$^{25}$INFN Sezione di Milano, Milano, Italy\\
$^{26}$INFN Sezione di Milano-Bicocca, Milano, Italy\\
$^{27}$INFN Sezione di Cagliari, Monserrato, Italy\\
$^{28}$Universit{\`a} degli Studi di Padova, Universit{\`a} e INFN, Padova, Padova, Italy\\
$^{29}$INFN Sezione di Pisa, Pisa, Italy\\
$^{30}$INFN Sezione di Roma La Sapienza, Roma, Italy\\
$^{31}$INFN Sezione di Roma Tor Vergata, Roma, Italy\\
$^{32}$Nikhef National Institute for Subatomic Physics, Amsterdam, Netherlands\\
$^{33}$Nikhef National Institute for Subatomic Physics and VU University Amsterdam, Amsterdam, Netherlands\\
$^{34}$AGH - University of Science and Technology, Faculty of Physics and Applied Computer Science, Krak{\'o}w, Poland\\
$^{35}$Henryk Niewodniczanski Institute of Nuclear Physics  Polish Academy of Sciences, Krak{\'o}w, Poland\\
$^{36}$National Center for Nuclear Research (NCBJ), Warsaw, Poland\\
$^{37}$Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest-Magurele, Romania\\
$^{38}$Affiliated with an institute covered by a cooperation agreement with CERN\\
$^{39}$ICCUB, Universitat de Barcelona, Barcelona, Spain\\
$^{40}$Instituto Galego de F{\'\i}sica de Altas Enerx{\'\i}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain\\
$^{41}$Instituto de Fisica Corpuscular, Centro Mixto Universidad de Valencia - CSIC, Valencia, Spain\\
$^{42}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$^{43}$Institute of Physics, Ecole Polytechnique  F{\'e}d{\'e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$^{44}$Physik-Institut, Universit{\"a}t Z{\"u}rich, Z{\"u}rich, Switzerland\\
$^{45}$NSC Kharkiv Institute of Physics and Technology (NSC KIPT), Kharkiv, Ukraine\\
$^{46}$Institute for Nuclear Research of the National Academy of Sciences (KINR), Kyiv, Ukraine\\
$^{47}$University of Birmingham, Birmingham, United Kingdom\\
$^{48}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom\\
$^{49}$Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom\\
$^{50}$Department of Physics, University of Warwick, Coventry, United Kingdom\\
$^{51}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$^{52}$School of Physics and Astronomy, University of Edinburgh, Edinburgh, United Kingdom\\
$^{53}$School of Physics and Astronomy, University of Glasgow, Glasgow, United Kingdom\\
$^{54}$Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom\\
$^{55}$Imperial College London, London, United Kingdom\\
$^{56}$Department of Physics and Astronomy, University of Manchester, Manchester, United Kingdom\\
$^{57}$Department of Physics, University of Oxford, Oxford, United Kingdom\\
$^{58}$Massachusetts Institute of Technology, Cambridge, MA, United States\\
$^{59}$University of Cincinnati, Cincinnati, OH, United States\\
$^{60}$University of Maryland, College Park, MD, United States\\
$^{61}$Los Alamos National Laboratory (LANL), Los Alamos, NM, United States\\
$^{62}$Syracuse University, Syracuse, NY, United States\\
$^{63}$School of Physics and Astronomy, Monash University, Melbourne, Australia, associated to $^{50}$\\
$^{64}$Pontif{\'\i}cia Universidade Cat{\'o}lica do Rio de Janeiro (PUC-Rio), Rio de Janeiro, Brazil, associated to $^{2}$\\
$^{65}$Physics and Micro Electronic College, Hunan University, Changsha City, China, associated to $^{7}$\\
$^{66}$Guangdong Provincial Key Laboratory of Nuclear Science, Guangdong-Hong Kong Joint Laboratory of Quantum Matter, Institute of Quantum Matter, South China Normal University, Guangzhou, China, associated to $^{3}$\\
$^{67}$School of Physics and Technology, Wuhan University, Wuhan, China, associated to $^{3}$\\
$^{68}$Departamento de Fisica , Universidad Nacional de Colombia, Bogota, Colombia, associated to $^{13}$\\
$^{69}$Universit{\"a}t Bonn - Helmholtz-Institut f{\"u}r Strahlen und Kernphysik, Bonn, Germany, associated to $^{17}$\\
$^{70}$Eotvos Lorand University, Budapest, Hungary, associated to $^{42}$\\
$^{71}$INFN Sezione di Perugia, Perugia, Italy, associated to $^{21}$\\
$^{72}$Van Swinderen Institute, University of Groningen, Groningen, Netherlands, associated to $^{32}$\\
$^{73}$Universiteit Maastricht, Maastricht, Netherlands, associated to $^{32}$\\
$^{74}$DS4DS, La Salle, Universitat Ramon Llull, Barcelona, Spain, associated to $^{39}$\\
$^{75}$Department of Physics and Astronomy, Uppsala University, Uppsala, Sweden, associated to $^{53}$\\
$^{76}$University of Michigan, Ann Arbor, MI, United States, associated to $^{62}$\\
\bigskip
$^{a}$Universidade Federal do Tri{\^a}ngulo Mineiro (UFTM), Uberaba-MG, Brazil\\
$^{b}$Central South U., Changsha, China\\
$^{c}$Hangzhou Institute for Advanced Study, UCAS, Hangzhou, China\\
$^{d}$Excellence Cluster ORIGINS, Munich, Germany\\
$^{e}$Universidad Nacional Aut{\'o}noma de Honduras, Tegucigalpa, Honduras\\
$^{f}$Universit{\`a} di Bari, Bari, Italy\\
$^{g}$Universit{\`a} di Bologna, Bologna, Italy\\
$^{h}$Universit{\`a} di Cagliari, Cagliari, Italy\\
$^{i}$Universit{\`a} di Ferrara, Ferrara, Italy\\
$^{j}$Universit{\`a} di Firenze, Firenze, Italy\\
$^{k}$Universit{\`a} di Genova, Genova, Italy\\
$^{l}$Universit{\`a} degli Studi di Milano, Milano, Italy\\
$^{m}$Universit{\`a} di Milano Bicocca, Milano, Italy\\
$^{n}$Universit{\`a} di Padova, Padova, Italy\\
$^{o}$Universit{\`a}  di Perugia, Perugia, Italy\\
$^{p}$Scuola Normale Superiore, Pisa, Italy\\
$^{q}$Universit{\`a} di Pisa, Pisa, Italy\\
$^{r}$Universit{\`a} della Basilicata, Potenza, Italy\\
$^{s}$Universit{\`a} di Roma Tor Vergata, Roma, Italy\\
$^{t}$Universit{\`a} di Siena, Siena, Italy\\
$^{u}$Universit{\`a} di Urbino, Urbino, Italy\\
\medskip
$ ^{\dagger}$Deceased
}
\end{flushleft}

==> LHCb_Authorship_DD-MMM-20YY.tex <==
% ===============================================================================
% Purpose: example of authorlist for LHCb template
% Author:
% Created on: 2009-09-24
% ===============================================================================

%\documentclass[a4paper]{article}
%\setlength{\oddsidemargin}{0cm}
%\setlength{\evensidemargin}{0cm}
%\setlength{\textwidth}{16.5cm}
%\setlength{\parindent}{0cm}
%\begin{document}
\centerline{\large\normalfont\bfseries LHCb collaboration}
\begin{flushleft}
\small
%-- LHCb Authorlist, Example typesetting
%-- 
A.~N.~Other$^{1}$.\bigskip\newline{\it
\footnotesize
$ ^{1}$University of nowhere\\
}
%-- 
%-- 
\end{flushleft}
%\end{document}




==> Makefile <==
# $Id: Makefile 87305 2016-02-08 13:50:32Z lafferty $
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN = main

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = template

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl
	BUILDCOMMANDUPRIGHT=rm -f upright.aux && $(LATEX) upright && bibtex upright && $(LATEX) upright && $(LATEX) upright
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && ./wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDUPRIGHT=rm -f upright.aux && $(LATEX) upright && bibtex upright && $(LATEX) upright && $(LATEX) upright && dvips -z -o upright.ps upright && ps2pdf upright.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

# list of all source files
TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib) $(wildcard *.bst)
FIGSOURCES = $(wildcard figs/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) $(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl $(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prl.pdf

# remove output file
rmout: 
	rm $(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl: 
	$(BUILDCOMMANDPRL)

# Make the PRL version
count: 
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo 

# Make the upright version
upright: 
	$(BUILDCOMMANDUPRIGHT)



==> acknowledgements_2022.tex <==
\section*{Acknowledgements}
%
% These Acknowledgements valid from 3-May-2019
%
\noindent We express our gratitude to our colleagues in the CERN
accelerator departments for the excellent performance of the LHC. We
thank the technical and administrative staff at the LHCb
institutes.
We acknowledge support from CERN and from the national agencies:
CAPES, CNPq, FAPERJ and FINEP (Brazil); 
MOST and NSFC (China); 
CNRS/IN2P3 (France); 
BMBF, DFG and MPG (Germany); 
INFN (Italy); 
NWO (Netherlands); 
MNiSW and NCN (Poland); 
MEN/IFA (Romania); 
%MSHE (Russia); 
MICINN (Spain); 
SNSF and SER (Switzerland); 
NASU (Ukraine); 
STFC (United Kingdom); 
DOE NP and NSF (USA).
We acknowledge the computing resources that are provided by CERN, IN2P3
(France), KIT and DESY (Germany), INFN (Italy), SURF (Netherlands),
PIC (Spain), GridPP (United Kingdom), 
%RRCKI and Yandex LLC (Russia), 
CSCS (Switzerland), IFIN-HH (Romania), CBPF (Brazil),
Polish WLCG  (Poland) and NERSC (USA).
We are indebted to the communities behind the multiple open-source
software packages on which we depend.
Individual groups or members have received support from
ARC and ARDC (Australia);
Minciencias (Colombia);
AvH Foundation (Germany);
EPLANET, Marie Sk\l{}odowska-Curie Actions and ERC (European Union);
A*MIDEX, ANR, IPhU and Labex P2IO, and R\'{e}gion Auvergne-Rh\^{o}ne-Alpes (France);
Key Research Program of Frontier Sciences of CAS, CAS PIFI, CAS CCEPP, 
Fundamental Research Funds for the Central Universities, 
and Sci. \& Tech. Program of Guangzhou (China);
%Key Research Program of Frontier Sciences of CAS, CAS PIFI,
%Thousand Talents Program, and Sci. \& Tech. Program of Guangzhou (China);
%RFBR, RSF and Yandex LLC (Russia);
GVA, XuntaGal, GENCAT and Prog.~Atracci\'on Talento, CM (Spain);
SRC (Sweden);
the Leverhulme Trust, the Royal Society
 and UKRI (United Kingdom).



==> body.tex <==
Measurements of $B$ mesons at colliders offer unique probes of the hadronization process by which single quarks evolve into color-neutral hadrons.  In contrast to light quarks, the large mass of $\bquark$ quarks suppresses their production via non-perturbative processes. In addition there is no $\bquark$ content in the valence quark distribution of the incoming beam particles \cite{Norrbin:2000zc}.  Therefore, production of $b\bar{b}$ pairs at hadron colliders is dominated by hard parton-parton interactions in the initial stages of the collisions, and is well described by perturbative QCD calculations \cite{LHCb-PAPER-2016-031,LHCb-PAPER-2017-037,ALICE:2021mgk}.  

The fraction of $\bquark$ quarks that pair with an $\squark$ quark to form $\Bs$ mesons, $f_{s}$, and the fraction that pair with a light $\dquark$ quark to form $\Bd$ mesons, $f_{d}$, are determined through the hadronization process.  One mechanism for hadronization is fragmentation, where showers of partons produced by outgoing quarks form into hadrons \cite{Andersson:1983ia,Webber:1983if}. Measurements of $B$ hadron production in $e^{+}e^{-}$ collisions at the $\Upsilonres(5S)$ \cite{CLEO:2005pyn,Belle:2006jvm,CLEO:2006dkk} and $Z^{0}$ \cite{OPAL:1992zsd, ALEPH:1995npv,L3:2000gcz, DELPHI:2003pao} resonances give consistent values for the ratio $f_{s}/f_{d}$, which is often interpreted as evidence for the universality of $\bquark$ quark fragmentation assumed by QCD factorization theorems \cite{Collins:1989gx}.  However, measurements at hadron colliders have shown that the ratio $f_{s}/f_{d}$ has a dependence on the collision center-of-mass energy and the $B$ meson transverse momentum $\pt$ \cite{CDF:1996ivk,LHCb-PAPER-2012-037, ATLAS:2015esn, LHCb-PAPER-2019-020,LHCb-PAPER-2020-046}. The fraction of $\bquark$ quarks which hadronize into baryons also varies with $\pt$ \cite{LHCb-PAPER-2011-018,LHCb-PAPER-2018-050}.  Additionally, recent measurements have shown that charm quark hadronization differs between $e^{+}e^{-}$ and $pp$ collisions \cite{ALICE:2021dhb}. The reason for these variations is not immediately clear, and may be explained by hadronization mechanisms other than fragmentation \cite{Berezhnoy:2013qln}.

An alternative hadronization process, quark coalescence, can occur when a quark produced in the collision combines with another quark to form a color singlet hadron.  Models incorporating coalescence are successful at reproducing a range of measurements from fixed-target experiments and colliders \cite{Vogt:1994zf,Braaten:2002yt,Rapp:2003wn,He:2019vgs,Minissale:2020bif}. Coalescence calculations generally require multiple quark wavefunctions to overlap in position and velocity, so the fraction of hadrons produced by this mechanism is expected to increase with the number of quarks produced in the collision.  The effect is expected to be most prominent at relatively low $\pt$, which is the range where the bulk of the particles created in the collision are found.  Coalescence can also lead to enhanced production of baryons at low $\pt$, and is especially important in high-energy heavy ion collisions where a large volume of deconfined quark-gluon plasma (QGP) is formed \cite{Fries:2003vb,Greco:2003xt,Molnar:2003ff}. Data from the CMS collaboration has shown that $\Bs$ production may be enhanced relative to $\Bu$ production in PbPb collisions when compared to $pp$ collisions \cite{CMS:2018eso,CMS:2021mzx}. However, significant uncertainties and the relatively high $\pt$ range covered by that data preclude drawing firm conclusions on the influence of coalescence on $B$ hadronization.

Recent measurements in $pp$ collisions have shown some behaviors similar to those associated with the formation of QGP in collisions of heavy nuclei \cite{CMS:2010ifv,ATLAS:2015hzw,CMS:2016fnw}.  Among these effects is an enhanced yield of light-quark baryons and mesons with strangeness in collisions where a relatively large number of charged particles are produced \cite{ALICE:2017jyt}, which was originally proposed as a QGP signature \cite{Koch:1986ud}.  If hadronization via coalescence emerges as a mechanism for forming final state $B$ hadrons, then the production rates of $\Bs$ hadrons could increase relative to the production of $\Bd$ hadrons as particle multiplicity increases. 

This Letter describes LHCb measurements of the ratio of $\Bs$ to $\Bd$ cross sections, $\sigma_{\Bs}/\sigma_{\Bd}$,  as a function of charged particle multiplicity and $\pt$.  Both the $\Bs$ and $\Bd$ candidates are reconstructed through their decays to the $\jpsi \pip \pim$ final state, where the $\jpsi$ decays into a $\mu^{+}\mu^{-}$ pair.  This decay mode provides similar yields for both $\Bs$ and $\Bd$ mesons.
Here multiplicity is represented by the number of charged tracks reconstructed in a silicon strip detector that surrounds the $pp$ interaction region, the LHCb VELO detector \cite{LHCb-TDR-005,LHCb-DP-2014-001}.  These measurements use a sample of $pp$ collisions collected at a center-of-mass energy $\sqrt{{s}} = 13\tev$, corresponding to an integrated luminosity of 5.4~fb$^{-1}$.

The LHCb detector is a single-arm forward spectrometer covering the pseudorapidity range $2 < \eta < 5$, described in detail in Refs.~\cite{LHCb-DP-2008-001,LHCb-DP-2014-002}.  Events considered in this analysis are required to satisfy a series of triggers designed to select the decay $\jpsi\rightarrow\mup\mu^{-}$ and have one reconstructed $pp$ interaction point (primary vertex).  Each muon candidate is required to penetrate the hadron absorber layers in the LHCb muon system and have $\pt> 500 \mevc$.  Candidate $\jpsi$ mesons are formed from pairs of oppositely charged muon candidates that have an invariant mass near the known $\jpsi$ mass and originate from a vertex that is displaced from the primary vertex.  Charged pion candidates are identified by the response of the LHCb ring-imaging Cherenkov detectors, and are required to have total momentum $p>3\gevc$ and transverse momentum $\pt>750\mevc$.  Candidate $\mup\mu^{-}\pip\pim$ combinations that form a good quality common vertex are retained, and the tracks are refit with kinematic constraints that fix the $\mup\mu^{-}$ invariant mass to the known $\jpsi$ mass, and require all four tracks to have the same origin point \cite{Hulsbergen:2005pu}.  

Simulation is required to model the effects of the detector acceptance and the selection requirements.  In the simulation, $pp$ collisions are generated using \pythia~\cite{Sjostrand:2007gs,*Sjostrand:2006za} with a specific \lhcb configuration~\cite{LHCb-PROC-2010-056}. Decays of unstable particles are described by \evtgen~\cite{Lange:2001uf}.  The interaction of the generated particles with the detector, and its response, are implemented using the \geant toolkit~\cite{Allison:2006ve, *Agostinelli:2002hh} as described in Ref.~\cite{LHCb-PROC-2011-006}. The $\pt$ distributions of the simulated $\Bs$ and $\Bd$ mesons, the invariant mass distributions of $\pip \pim$ pairs from their decays, and simulated event multiplicity distributions are weighted to match background-subtracted distributions that are extracted from the data using the \sPlot method \cite{splot}. 

The multiplicity metrics used in this analysis are the total number of charged tracks reconstructed in the VELO detector, $\Nvelo$, and the subset of VELO tracks that point in the backward direction, away from the LHCb spectrometer, $\Nback$.  The backward tracks cover a pseudorapidity interval of approximately $-3.5<\eta<-1.5$, providing a multiplicity estimate that is measured in a different region than the signal.  The VELO detector and its performance are described in detail in Refs. \cite{LHCb-TDR-005,LHCb-DP-2014-001}.  Figure \ref{fig:Fig1} shows the distributions of $\Nvelo$ and $\Nback$ for both NoBias events and $\Bd$ signal events with one reconstructed primary vertex, which requires at least five reconstructed tracks. NoBias events are selected based on the Large Hadron Collider beam clock, which indicates that a bunch crossing has occurred, without any other trigger requirements.  The distributions for $\Bd$ signal events are extracted from the data, and background is removed using the \sPlot method \cite{splot}.  The results are quoted in terms of normalized multiplicity, defined as the number of tracks at the center of a given multiplicity interval divided by the mean number of tracks in NoBias events, which are $\langle \Nvelo \rangle$$_{\mathrm{NoBias}}$ = 37.7 and $\langle \Nback \rangle$$_{\mathrm{NoBias}}$ = 11.1, with negligibly small uncertainties.  For comparison, the mean number of $\Nvelo$ and $\Nback$ are $71.1\pm0.1$ and $17.4\pm0.3$ for $\Bd$ signal events, respectively, where the uncertainty is due to the statistical uncertainty on the track distributions.  In some respects, the low- and high-multiplicity data samples approach the hadronic environments achieved in $e^{+}e^{-}$ collisions and heavy-ion collisions, respectively.


 \begin{figure}[!ht]
  \centering
  \includegraphics[width=0.7\linewidth]{./back_velo_mult_compare.pdf}
  \caption{Distribution of the number of VELO tracks and backward tracks for NoBias events (red) and $\Bd$ signal events (blue), each with only one primary vertex. The vertical scale is arbitrary.}
  \label{fig:Fig1}
\end{figure}
%/Users/durham/Documents/LHCb/Bs/NoBias/draw_nvelo_nback.C

The sample containing signal events is divided into intervals of multiplicity, and in each interval a likelihood fit is performed on the $\jpsi \pip \pim$ invariant mass spectrum to determine the ratio of $\Bs$ to $\Bd$ yields.  Examples of the $\jpsi \pip \pim$ mass distribution in low- and high-multiplicity intervals are shown in Fig. \ref{fig:Bs_fit_example}.  An increase of the $\Bs$ yield relative to the $\Bd$ yield in the high-multiplicity interval is apparent.  The $\Bs$ and $\Bd$ peaks are each represented in the fit by a sum of two Crystal Ball functions, which have tail parameters constrained to values determined by simulation.  The background contribution is represented by an exponential function, which is found to provide a good description of the purely combinatorial $\jpsi \pi^{\pm} \pi^{\pm}$ mass spectrum with like-sign dipions.  All multiplicity intervals are fit simultaneously, where the signal shapes are constrained to be the same in each interval, but their normalization and the background parameters are allowed to vary.  The $\Bs$ and $\Bd$ line shapes are nearly identical, and variations of the fit functions have a negligible effect on the extracted ratio of $\Bs$ to $\Bd$ yields. 

 \begin{figure}[b]
  \centering
  \includegraphics[width=1.0\linewidth]{./Fig2.pdf}
  \caption{Measured $\jpsi \pip \pim$ invariant mass distributions and fit projections in the multiplicity ranges a) $30<\Nvelo\leq40$ and b) $100<\Nvelo\leq125$.}
  \label{fig:Bs_fit_example}
\end{figure}
%/Users/durham/Documents/LHCb/Bs/fit/simult_pt_Bsfit.C

 The ratio of cross-sections $\sigma_{\Bs}/\sigma_{\Bd}$ is found by calculating
%
\begin{equation}
\label{eqn:rat}
\begin{aligned}
\frac{\sigma_{\Bs}}{\sigma_{\Bd}} = \frac{N_{\Bs}}{N_{\Bd}} \times
\frac{\BR_{\Bd}}{\BR_{\Bs}} \times
\frac{\varepsilon_{\Bd}^{\mathrm{acc}}}{\varepsilon_{\Bs}^{\mathrm{acc}}} \times
\frac{\varepsilon_{\Bd}^{\mathrm{trig}}}{\varepsilon_{\Bs}^{\mathrm{trig}}} \times
\frac{\varepsilon_{\Bd}^{\mathrm{PID}}}{\varepsilon_{\Bs}^{\mathrm{PID}}} \times
\frac{\varepsilon_{\Bd}^{\mathrm{reco}}}{\varepsilon_{\Bs}^{\mathrm{reco}}},\\
\end{aligned}
\end{equation}
%
where $N_{\Bs}/N_{\Bd}$ is the ratio of $\Bs$ to $\Bd$ signal yields returned by the fit, $\BR_{\Bd}/\BR_{\Bs}$ is the ratio of $\Bd$ to $\Bs$ branching fractions to $\jpsi \pip \pim$ \cite{ParticleDataGroup:2020ssz,LHCb-PAPER-2020-046}, and $\varepsilon_{\Bd}^{\mathrm{acc}}/\varepsilon_{\Bs}^{\mathrm{acc}},
\varepsilon_{\Bd}^{\mathrm{trig}}/\varepsilon_{\Bs}^{\mathrm{trig}},
\varepsilon_{\Bd}^{\mathrm{PID}}/\varepsilon_{\Bs}^{\mathrm{PID}}$, and  $\varepsilon_{\Bd}^{\mathrm{reco}}/\varepsilon_{\Bs}^{\mathrm{reco}}$ are ratios of the LHCb acceptance and the trigger, particle identification, and reconstruction efficiencies for $\Bd$ to $\Bs$ mesons, respectively.  Due to the similarities of the $\Bs$ and $\Bd$ decays, many systematic uncertainties partially cancel in this ratio of cross sections.  The ratio of the LHCb acceptance for the decays $\varepsilon_{\Bd}^{\mathrm{acc}}/\varepsilon_{\Bs}^{\mathrm{acc}}$ is found, using simulation, to be consistent with unity, with an uncertainty of $\sim1\%$ due to the uncertainty on the weights applied to the simulation in order to match the data.  The ratio of trigger efficiencies $\varepsilon_{\Bd}^{\mathrm{trig}}/\varepsilon_{\Bs}^{\mathrm{trig}}$ is determined from data to be consistent with unity, with an uncertainty of $\sim1\%$, using techniques described in Ref. \cite{LHCb-PUB-2014-039}, where the uncertainty comes from statistical uncertainties on the data sample. The ratio of particle identification efficiencies $\varepsilon_{\Bd}^{\mathrm{PID}}/\varepsilon_{\Bs}^{\mathrm{PID}}$ is found using calibrated samples of identified muons and pions obtained from the data, and is consistent with unity with an uncertainty of $\sim1\%$ due to the finite size of the calibration sample.  The only term with a significant difference from unity is the ratio of reconstruction efficiencies, which is found to be \mbox{ $\varepsilon_{\Bd}^{\mathrm{reco}}/\varepsilon_{\Bs}^{\mathrm{reco}}$ = $0.86\pm0.04$} for the $\pt$-integrated sample.  This is due to the difference in the dipion mass distributions produced in the $\Bs$ and $\Bd$ decays: the $\Bs$ decay is dominated by contributions from intermediate $f_{0}(980)$ and $f_{0}(1500)$ states \cite{LHCb-PAPER-2013-069}, which are reconstructed with higher efficiency than the lower-mass $\rho^{0}(770)$ intermediate state that is significant in $\Bd$ decays \cite{LHCb-PAPER-2014-012}.  The uncertainty on this correction is due to the statistical uncertainty on the weights extracted from the data that are applied to the simulation in order to match the measured $B$ meson $\pt$ and dipion mass distributions.



The ratio of cross-sections for the multiplicity-integrated samples is found to be $\sigma_{\Bs}/\sigma_{\Bd} = 0.30\pm 0.01\pm 0.03$, where the first uncertainty is statistical and the second is systematic.  This measurement agrees with previous LHCb measurements of $f_{s}/f_{d}$ using different decay channels \cite{LHCb-PAPER-2020-046} within $1.5$ standard deviations.  



The multiplicity dependence of $\sigma_{\Bs}/\sigma_{\Bd}$ is shown in Fig. \ref{fig:Fig3}, for two different multiplicity metrics.  The vertical error bars (boxes) represent point-to-point uncorrelated (fully correlated) uncertainties, while the horizontal error bars represent the bin width.  Numerical values are given in the supplemental material~\cite{ref:SuppMat}.  In the left panel, the ratio shows an increasing trend with the total VELO multiplicity, where multiplicity is normalized to the mean value found in NoBias collisions.  Also shown are the $\sigma_{\Bs}/\sigma_{\Bd}$ values measured in $e^{+}e^{-}$ collisions at the $\Upsilonres(5S)$ and $Z^{0}$ resonances \cite{HFLAV:2019otj}, which are in good agreement with the data at low multiplicity.  The right panel shows the same ratio versus the normalized $\Nback$.  No significant dependence is observed on the multiplicity measured in the backward region. The dependence on total multiplicity, compared to the lack of dependence on multiplicity measured at backward rapidity, could indicate that the mechanism responsible for the increase in the $\sigma_{\Bs}/\sigma_{\Bd}$ ratio is related to the local particle density in a similar rapidity interval as the $B$ mesons themselves.

\begin{figure}[b]
  \centering
  \includegraphics[width=0.8\linewidth]{./Fig3.pdf}
  \caption{Ratio of cross sections $\sigma_{\Bs}/\sigma_{\Bd}$ versus the normalized multiplicity of a) all VELO tracks, and b) backward VELO tracks.  The vertical error bars (boxes) represent point-to-point uncorrelated (fully correlated) uncertainties.  The horizontal bands show the values measured in $e^{+}e^{-}$ collisions.}
  \label{fig:Fig3}
\end{figure}

The multiplicity dependence of $\sigma_{\Bs}/\sigma_{\Bd}$ is shown in three different intervals of $B$ meson $\pt$ in Fig. \ref{fig:Fig4}.  Numerical values are given in the supplemental material~\cite{ref:SuppMat}.  The lowest $\pt$ interval, $0<\pt<6$ GeV/$c$, encompasses $B$ mesons with $\pt$ approximately equal to or less than their mass.  In this $\pt$ interval, at low multiplicity the $\sigma_{\Bs}/\sigma_{\Bd}$ ratio is consistent with values measured in $e^{+}e^{-}$ collisions, and increases with multiplicity. A line fit to these data returns a slope of $0.075\pm0.022$ $(\Nvelo /\langle \Nvelo \rangle_{\mathrm{NoBias}})^{-1}$, which differs from zero by 3.4 standard deviations and thereby provides evidence for an increase of the the $\sigma_{\Bs}/\sigma_{\Bd}$ ratio. This fit considers only the point-to-point uncorrelated uncertainties; since all data points must move simultaneously within the correlated uncertainties, they have no effect on the extracted slope.

For comparison, the ratio of cross sections calculated by the PYTHIA event generator is also shown.  Events are generated with and without color reconnection (CR), a process which allows partons produced by from different interactions in the collision to be connected by color lines \cite{Sjostrand:1987su,Sjostrand:2013cya}.  Color reconnection was introduced to model charged particle production in hadron collisions, and is thought to be especially important in high-multiplicity collisions where multiple-parton interactions are significant.  Both sets of PYTHIA calculations show a rise with multiplicity,  which is more pronounced when CR is included.  The PYTHIA models agree with the data at relatively low multiplicity, but both scenarios give values that are lower than the central values of the data at high multiplicity.

The measurements in higher $\pt$ intervals, $6<\pt<12$ GeV/$c$ and $12<\pt<20$ GeV/$c$, display no significant dependence on multiplicity and are consistent with data from $e^{+}e^{-}$ collisions.  This behavior is expected in a scenario where low-$\pt$ $\bquark$ quarks with relatively low velocity recombine with $s$ quarks produced in high-multiplicity collisions, while the wavefunctions of higher $\pt$ $\bquark$ quarks have less overlap with the low-$\pt$ bulk of the quarks produced in the collision.  These high-$\pt$ $\bquark$ quarks would thereby dominantly hadronize via fragmentation in vacuum, as in $e^{+}e^{-}$ collisions, rather than via coalescence.  Again, both sets of PYTHIA calculations show a rising trend, which is more pronounced when color reconnection is included.  However, here the uncertainties on the data prevent discrimination between the two scenarios.  Lines fit to the $6<\pt<12$ GeV/$c$ and $12<\pt<20$ GeV/$c$ data have slopes that are consistent with zero within 0.2 and 1.3 standard deviations, respectively.

\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{./Fig4.pdf}
  \caption{Ratio of cross sections $\sigma_{\Bs}/\sigma_{\Bd}$ versus normalized multiplicity in the transverse momentum ranges a) $0<\pt<6$ GeV/$c$, b) $6<\pt<12$ GeV/$c$, and c) $12<\pt<20$ GeV/$c$.  The vertical error bars (boxes) represent point-to-point uncorrelated (fully correlated) uncertainties.  The horizontal bands show the values measured in $e^{+}e^{-}$ collisions and the horizontal lines show PYTHIA calculations with and without (w/o) color reconnection.}
  \label{fig:Fig4}
\end{figure}

In summary, LHCb measurements in $pp$ collisions at $\sqs$ = 13\tev show evidence that the production of $\Bs$ mesons is enhanced relative to $\Bd$ mesons in collisions with high charged-particle multiplicity, indicating that strangeness enhancement is present in $B$ hadron production.  In collisions with relatively low charged-particle multiplicity, and for $B$ mesons with $\pt>6$ GeV/$c$, the rate of $\Bs$ production relative to $\Bd$ production is consistent with what is measured in $e^+e^-$ collisions.  These measurements are qualitatively consistent with expectations based on the emergence of quark coalescence as an additional hadronization mechanism, rather than fragmentation alone.  These results could indicate that interactions of the $\bquark$ quarks with the local hadronic environment influence the hadronization process, thereby breaking factorization of $\bquark$ quark hadronization between $e^{+}e^{-}$ and hadron collisions.




==> justification.tex <==
\clearpage

\section{PRL justification}
\label{sec:justification}

Factorization theorems in QCD assume that quark fragmentation is a universal process, independent of collision system.  Differences in $b$ quark fragmentation measured at $e^{+}e^{-}$ colliders versus hadron colliders are thereby unexpected, and remain unexplained.  This measurement leverages LHCb’s unique capabilities and strangeness enhancement techniques adapted from heavy-ion physics to bridge the gap between $b\overline{b}$ production in vacuum (approximated by low multiplicity collisions) and production in a dense hadronic environment (high multiplicity collisions).  The results provide important new insight into fundamental mechanisms by which single quarks form into color-neutral matter and are thereby relevant to all areas of QCD.  

\clearpage


==> lhcb-symbols-list.tex <==
% This is an automatically generated appendix to template.tex. 
% When included it will show all the symbols defined in lhcb-symbols-def.tex.
%
% To regenerate with the latest definitions run the script python listsymbols.py

\section{List of all symbols}
\label{sec:listofsymbols}
\subsection{Experiments}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash lhcb} & \lhcb & \texttt{\textbackslash atlas} & \atlas & \texttt{\textbackslash cms} & \cms \\
\texttt{\textbackslash alice} & \alice & \texttt{\textbackslash babar} & \babar & \texttt{\textbackslash belle} & \belle \\
\texttt{\textbackslash belletwo} & \belletwo & \texttt{\textbackslash besiii} & \besiii & \texttt{\textbackslash cleo} & \cleo \\
\texttt{\textbackslash cdf} & \cdf & \texttt{\textbackslash dzero} & \dzero & \texttt{\textbackslash aleph} & \aleph \\
\texttt{\textbackslash delphi} & \delphi & \texttt{\textbackslash opal} & \opal & \texttt{\textbackslash lthree} & \lthree \\
\texttt{\textbackslash sld} & \sld & \texttt{\textbackslash cern} & \cern & \texttt{\textbackslash lhc} & \lhc \\
\texttt{\textbackslash lep} & \lep & \texttt{\textbackslash tevatron} & \tevatron & \texttt{\textbackslash bfactories} & \bfactories \\
\texttt{\textbackslash bfactory} & \bfactory & \texttt{\textbackslash upgradeone} & \upgradeone & \texttt{\textbackslash upgradetwo} & \upgradetwo \\
\end{tabular*}

\subsubsection{LHCb sub-detectors and sub-systems}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash velo} & \velo & \texttt{\textbackslash rich} & \rich & \texttt{\textbackslash richone} & \richone \\
\texttt{\textbackslash richtwo} & \richtwo & \texttt{\textbackslash ttracker} & \ttracker & \texttt{\textbackslash intr} & \intr \\
\texttt{\textbackslash st} & \st & \texttt{\textbackslash ot} & \ot & \texttt{\textbackslash herschel} & \herschel \\
\texttt{\textbackslash spd} & \spd & \texttt{\textbackslash presh} & \presh & \texttt{\textbackslash ecal} & \ecal \\
\texttt{\textbackslash hcal} & \hcal & \texttt{\textbackslash MagUp} & \MagUp & \texttt{\textbackslash MagDown} & \MagDown \\
\texttt{\textbackslash ode} & \ode & \texttt{\textbackslash daq} & \daq & \texttt{\textbackslash tfc} & \tfc \\
\texttt{\textbackslash ecs} & \ecs & \texttt{\textbackslash lone} & \lone & \texttt{\textbackslash hlt} & \hlt \\
\texttt{\textbackslash hltone} & \hltone & \texttt{\textbackslash hlttwo} & \hlttwo &  \\
\end{tabular*}

\subsection{Particles}
\subsubsection{Leptons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash electron} & \electron & \texttt{\textbackslash en} & \en & \texttt{\textbackslash ep} & \ep \\
\texttt{\textbackslash epm} & \epm & \texttt{\textbackslash emp} & \emp & \texttt{\textbackslash epem} & \epem \\
\texttt{\textbackslash muon} & \muon & \texttt{\textbackslash mup} & \mup & \texttt{\textbackslash mun} & \mun \\
\texttt{\textbackslash mupm} & \mupm & \texttt{\textbackslash mump} & \mump & \texttt{\textbackslash mumu} & \mumu \\
\texttt{\textbackslash tauon} & \tauon & \texttt{\textbackslash taup} & \taup & \texttt{\textbackslash taum} & \taum \\
\texttt{\textbackslash taupm} & \taupm & \texttt{\textbackslash taump} & \taump & \texttt{\textbackslash tautau} & \tautau \\
\texttt{\textbackslash lepton} & \lepton & \texttt{\textbackslash ellm} & \ellm & \texttt{\textbackslash ellp} & \ellp \\
\texttt{\textbackslash ellpm} & \ellpm & \texttt{\textbackslash ellmp} & \ellmp & \texttt{\textbackslash ellell} & \ellell \\
\texttt{\textbackslash neu} & \neu & \texttt{\textbackslash neub} & \neub & \texttt{\textbackslash neue} & \neue \\
\texttt{\textbackslash neueb} & \neueb & \texttt{\textbackslash neum} & \neum & \texttt{\textbackslash neumb} & \neumb \\
\texttt{\textbackslash neut} & \neut & \texttt{\textbackslash neutb} & \neutb & \texttt{\textbackslash neul} & \neul \\
\texttt{\textbackslash neulb} & \neulb &  \\
\end{tabular*}

\subsubsection{Gauge bosons and scalars}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash g} & \g & \texttt{\textbackslash H} & \H & \texttt{\textbackslash Hp} & \Hp \\
\texttt{\textbackslash Hm} & \Hm & \texttt{\textbackslash Hpm} & \Hpm & \texttt{\textbackslash W} & \W \\
\texttt{\textbackslash Wp} & \Wp & \texttt{\textbackslash Wm} & \Wm & \texttt{\textbackslash Wpm} & \Wpm \\
\texttt{\textbackslash Z} & \Z &  \\
\end{tabular*}

\subsubsection{Quarks}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash quark} & \quark & \texttt{\textbackslash quarkbar} & \quarkbar & \texttt{\textbackslash qqbar} & \qqbar \\
\texttt{\textbackslash uquark} & \uquark & \texttt{\textbackslash uquarkbar} & \uquarkbar & \texttt{\textbackslash uubar} & \uubar \\
\texttt{\textbackslash dquark} & \dquark & \texttt{\textbackslash dquarkbar} & \dquarkbar & \texttt{\textbackslash ddbar} & \ddbar \\
\texttt{\textbackslash squark} & \squark & \texttt{\textbackslash squarkbar} & \squarkbar & \texttt{\textbackslash ssbar} & \ssbar \\
\texttt{\textbackslash cquark} & \cquark & \texttt{\textbackslash cquarkbar} & \cquarkbar & \texttt{\textbackslash ccbar} & \ccbar \\
\texttt{\textbackslash bquark} & \bquark & \texttt{\textbackslash bquarkbar} & \bquarkbar & \texttt{\textbackslash bbbar} & \bbbar \\
\texttt{\textbackslash tquark} & \tquark & \texttt{\textbackslash tquarkbar} & \tquarkbar & \texttt{\textbackslash ttbar} & \ttbar \\
\end{tabular*}

\subsubsection{Light mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash hadron} & \hadron & \texttt{\textbackslash pion} & \pion & \texttt{\textbackslash piz} & \piz \\
\texttt{\textbackslash pip} & \pip & \texttt{\textbackslash pim} & \pim & \texttt{\textbackslash pipm} & \pipm \\
\texttt{\textbackslash pimp} & \pimp & \texttt{\textbackslash rhomeson} & \rhomeson & \texttt{\textbackslash rhoz} & \rhoz \\
\texttt{\textbackslash rhop} & \rhop & \texttt{\textbackslash rhom} & \rhom & \texttt{\textbackslash rhopm} & \rhopm \\
\texttt{\textbackslash rhomp} & \rhomp & \texttt{\textbackslash kaon} & \kaon & \texttt{\textbackslash Kbar} & \Kbar \\
\texttt{\textbackslash Kb} & \Kb & \texttt{\textbackslash KorKbar} & \KorKbar & \texttt{\textbackslash Kz} & \Kz \\
\texttt{\textbackslash Kzb} & \Kzb & \texttt{\textbackslash Kp} & \Kp & \texttt{\textbackslash Km} & \Km \\
\texttt{\textbackslash Kpm} & \Kpm & \texttt{\textbackslash Kmp} & \Kmp & \texttt{\textbackslash KS} & \KS \\
\texttt{\textbackslash Vzero} & \Vzero & \texttt{\textbackslash KL} & \KL & \texttt{\textbackslash Kstarz} & \Kstarz \\
\texttt{\textbackslash Kstarzb} & \Kstarzb & \texttt{\textbackslash Kstar} & \Kstar & \texttt{\textbackslash Kstarb} & \Kstarb \\
\texttt{\textbackslash Kstarp} & \Kstarp & \texttt{\textbackslash Kstarm} & \Kstarm & \texttt{\textbackslash Kstarpm} & \Kstarpm \\
\texttt{\textbackslash Kstarmp} & \Kstarmp & \texttt{\textbackslash KorKbarz} & \KorKbarz & \texttt{\textbackslash etaz} & \etaz \\
\texttt{\textbackslash etapr} & \etapr & \texttt{\textbackslash phiz} & \phiz & \texttt{\textbackslash omegaz} & \omegaz \\
\end{tabular*}

\subsubsection{Charmed mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Dbar} & \Dbar & \texttt{\textbackslash D} & \D & \texttt{\textbackslash Db} & \Db \\
\texttt{\textbackslash DorDbar} & \DorDbar & \texttt{\textbackslash Dz} & \Dz & \texttt{\textbackslash Dzb} & \Dzb \\
\texttt{\textbackslash Dp} & \Dp & \texttt{\textbackslash Dm} & \Dm & \texttt{\textbackslash Dpm} & \Dpm \\
\texttt{\textbackslash Dmp} & \Dmp & \texttt{\textbackslash DpDm} & \DpDm & \texttt{\textbackslash Dstar} & \Dstar \\
\texttt{\textbackslash Dstarb} & \Dstarb & \texttt{\textbackslash Dstarz} & \Dstarz & \texttt{\textbackslash Dstarzb} & \Dstarzb \\
\texttt{\textbackslash theDstarz} & \theDstarz & \texttt{\textbackslash theDstarzb} & \theDstarzb & \texttt{\textbackslash Dstarp} & \Dstarp \\
\texttt{\textbackslash Dstarm} & \Dstarm & \texttt{\textbackslash Dstarpm} & \Dstarpm & \texttt{\textbackslash Dstarmp} & \Dstarmp \\
\texttt{\textbackslash theDstarp} & \theDstarp & \texttt{\textbackslash theDstarm} & \theDstarm & \texttt{\textbackslash theDstarpm} & \theDstarpm \\
\texttt{\textbackslash theDstarmp} & \theDstarmp & \texttt{\textbackslash Ds} & \Ds & \texttt{\textbackslash Dsp} & \Dsp \\
\texttt{\textbackslash Dsm} & \Dsm & \texttt{\textbackslash Dspm} & \Dspm & \texttt{\textbackslash Dsmp} & \Dsmp \\
\texttt{\textbackslash Dss} & \Dss & \texttt{\textbackslash Dssp} & \Dssp & \texttt{\textbackslash Dssm} & \Dssm \\
\texttt{\textbackslash Dsspm} & \Dsspm & \texttt{\textbackslash Dssmp} & \Dssmp & \texttt{\textbackslash DporDsp} & \DporDsp \\
\texttt{\textbackslash DmorDsm} & \DmorDsm & \texttt{\textbackslash DpmorDspm} & \DpmorDspm &  \\
\end{tabular*}

\subsubsection{Beauty mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash B} & \B & \texttt{\textbackslash Bbar} & \Bbar & \texttt{\textbackslash Bb} & \Bb \\
\texttt{\textbackslash BorBbar} & \BorBbar & \texttt{\textbackslash Bz} & \Bz & \texttt{\textbackslash Bzb} & \Bzb \\
\texttt{\textbackslash Bd} & \Bd & \texttt{\textbackslash Bdb} & \Bdb & \texttt{\textbackslash BdorBdbar} & \BdorBdbar \\
\texttt{\textbackslash Bu} & \Bu & \texttt{\textbackslash Bub} & \Bub & \texttt{\textbackslash Bp} & \Bp \\
\texttt{\textbackslash Bm} & \Bm & \texttt{\textbackslash Bpm} & \Bpm & \texttt{\textbackslash Bmp} & \Bmp \\
\texttt{\textbackslash Bs} & \Bs & \texttt{\textbackslash Bsb} & \Bsb & \texttt{\textbackslash BsorBsbar} & \BsorBsbar \\
\texttt{\textbackslash Bc} & \Bc & \texttt{\textbackslash Bcp} & \Bcp & \texttt{\textbackslash Bcm} & \Bcm \\
\texttt{\textbackslash Bcpm} & \Bcpm & \texttt{\textbackslash Bds} & \Bds & \texttt{\textbackslash Bdsb} & \Bdsb \\
\texttt{\textbackslash BdorBs} & \BdorBs & \texttt{\textbackslash BdorBsbar} & \BdorBsbar &  \\
\end{tabular*}

\subsubsection{Onia}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash jpsi} & \jpsi & \texttt{\textbackslash psitwos} & \psitwos & \texttt{\textbackslash psiprpr} & \psiprpr \\
\texttt{\textbackslash etac} & \etac & \texttt{\textbackslash psires} & \psires & \texttt{\textbackslash chic} & \chic \\
\texttt{\textbackslash chiczero} & \chiczero & \texttt{\textbackslash chicone} & \chicone & \texttt{\textbackslash chictwo} & \chictwo \\
\texttt{\textbackslash chicJ} & \chicJ & \texttt{\textbackslash Upsilonres} & \Upsilonres & \texttt{\textbackslash OneS} & \OneS \\
\texttt{\textbackslash TwoS} & \TwoS & \texttt{\textbackslash ThreeS} & \ThreeS & \texttt{\textbackslash FourS} & \FourS \\
\texttt{\textbackslash FiveS} & \FiveS & \texttt{\textbackslash chib} & \chib & \texttt{\textbackslash chibzero} & \chibzero \\
\texttt{\textbackslash chibone} & \chibone & \texttt{\textbackslash chibtwo} & \chibtwo & \texttt{\textbackslash chibJ} & \chibJ \\
\texttt{\textbackslash theX} & \theX &  \\
\end{tabular*}

\subsubsection{Light Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash proton} & \proton & \texttt{\textbackslash antiproton} & \antiproton & \texttt{\textbackslash neutron} & \neutron \\
\texttt{\textbackslash antineutron} & \antineutron & \texttt{\textbackslash Deltares} & \Deltares & \texttt{\textbackslash Deltaresbar} & \Deltaresbar \\
\texttt{\textbackslash Lz} & \Lz & \texttt{\textbackslash Lbar} & \Lbar & \texttt{\textbackslash LorLbar} & \LorLbar \\
\texttt{\textbackslash Lambdares} & \Lambdares & \texttt{\textbackslash Lambdaresbar} & \Lambdaresbar & \texttt{\textbackslash Sigmares} & \Sigmares \\
\texttt{\textbackslash Sigmaz} & \Sigmaz & \texttt{\textbackslash Sigmap} & \Sigmap & \texttt{\textbackslash Sigmam} & \Sigmam \\
\texttt{\textbackslash Sigmaresbar} & \Sigmaresbar & \texttt{\textbackslash Sigmabarz} & \Sigmabarz & \texttt{\textbackslash Sigmabarp} & \Sigmabarp \\
\texttt{\textbackslash Sigmabarm} & \Sigmabarm & \texttt{\textbackslash Xires} & \Xires & \texttt{\textbackslash Xiz} & \Xiz \\
\texttt{\textbackslash Xim} & \Xim & \texttt{\textbackslash Xiresbar} & \Xiresbar & \texttt{\textbackslash Xibarz} & \Xibarz \\
\texttt{\textbackslash Xibarp} & \Xibarp & \texttt{\textbackslash Omegares} & \Omegares & \texttt{\textbackslash Omegaresbar} & \Omegaresbar \\
\texttt{\textbackslash Omegam} & \Omegam & \texttt{\textbackslash Omegabarp} & \Omegabarp &  \\
\end{tabular*}

\subsubsection{Charmed Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Lc} & \Lc & \texttt{\textbackslash Lcbar} & \Lcbar & \texttt{\textbackslash Xic} & \Xic \\
\texttt{\textbackslash Xicz} & \Xicz & \texttt{\textbackslash Xicp} & \Xicp & \texttt{\textbackslash Xicbar} & \Xicbar \\
\texttt{\textbackslash Xicbarz} & \Xicbarz & \texttt{\textbackslash Xicbarm} & \Xicbarm & \texttt{\textbackslash Omegac} & \Omegac \\
\texttt{\textbackslash Omegacbar} & \Omegacbar & \texttt{\textbackslash Xicc} & \Xicc & \texttt{\textbackslash Xiccbar} & \Xiccbar \\
\texttt{\textbackslash Xiccp} & \Xiccp & \texttt{\textbackslash Xiccpp} & \Xiccpp & \texttt{\textbackslash Xiccbarm} & \Xiccbarm \\
\texttt{\textbackslash Xiccbarmm} & \Xiccbarmm & \texttt{\textbackslash Omegacc} & \Omegacc & \texttt{\textbackslash Omegaccbar} & \Omegaccbar \\
\texttt{\textbackslash Omegaccc} & \Omegaccc & \texttt{\textbackslash Omegacccbar} & \Omegacccbar &  \\
\end{tabular*}

\subsubsection{Beauty Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Lb} & \Lb & \texttt{\textbackslash Lbbar} & \Lbbar & \texttt{\textbackslash Sigmab} & \Sigmab \\
\texttt{\textbackslash Sigmabp} & \Sigmabp & \texttt{\textbackslash Sigmabz} & \Sigmabz & \texttt{\textbackslash Sigmabm} & \Sigmabm \\
\texttt{\textbackslash Sigmabpm} & \Sigmabpm & \texttt{\textbackslash Sigmabbar} & \Sigmabbar & \texttt{\textbackslash Sigmabbarp} & \Sigmabbarp \\
\texttt{\textbackslash Sigmabbarz} & \Sigmabbarz & \texttt{\textbackslash Sigmabbarm} & \Sigmabbarm & \texttt{\textbackslash Sigmabbarpm} & \Sigmabbarpm \\
\texttt{\textbackslash Xib} & \Xib & \texttt{\textbackslash Xibz} & \Xibz & \texttt{\textbackslash Xibm} & \Xibm \\
\texttt{\textbackslash Xibbar} & \Xibbar & \texttt{\textbackslash Xibbarz} & \Xibbarz & \texttt{\textbackslash Xibbarp} & \Xibbarp \\
\texttt{\textbackslash Omegab} & \Omegab & \texttt{\textbackslash Omegabbar} & \Omegabbar &  \\
\end{tabular*}

\subsection{Physics symbols}
\subsubsection{Decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BF} & \BF & \texttt{\textbackslash BR} & \BR & \texttt{\textbackslash BRvis} & \BRvis \\
\texttt{\textbackslash ra} & \ra & \texttt{\textbackslash to} & \to &  \\
\end{tabular*}

\subsubsection{Lifetimes}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tauBs} & \tauBs & \texttt{\textbackslash tauBd} & \tauBd & \texttt{\textbackslash tauBz} & \tauBz \\
\texttt{\textbackslash tauBu} & \tauBu & \texttt{\textbackslash tauDp} & \tauDp & \texttt{\textbackslash tauDz} & \tauDz \\
\texttt{\textbackslash tauL} & \tauL & \texttt{\textbackslash tauH} & \tauH &  \\
\end{tabular*}

\subsubsection{Masses}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash mBd} & \mBd & \texttt{\textbackslash mBp} & \mBp & \texttt{\textbackslash mBs} & \mBs \\
\texttt{\textbackslash mBc} & \mBc & \texttt{\textbackslash mLb} & \mLb &  \\
\end{tabular*}

\subsubsection{EW theory, groups}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash grpsuthree} & \grpsuthree & \texttt{\textbackslash grpsutw} & \grpsutw & \texttt{\textbackslash grpuone} & \grpuone \\
\texttt{\textbackslash ssqtw} & \ssqtw & \texttt{\textbackslash csqtw} & \csqtw & \texttt{\textbackslash stw} & \stw \\
\texttt{\textbackslash ctw} & \ctw & \texttt{\textbackslash ssqtwef} & \ssqtwef & \texttt{\textbackslash csqtwef} & \csqtwef \\
\texttt{\textbackslash stwef} & \stwef & \texttt{\textbackslash ctwef} & \ctwef & \texttt{\textbackslash gv} & \gv \\
\texttt{\textbackslash ga} & \ga & \texttt{\textbackslash order} & \order & \texttt{\textbackslash ordalph} & \ordalph \\
\texttt{\textbackslash ordalsq} & \ordalsq & \texttt{\textbackslash ordalcb} & \ordalcb &  \\
\end{tabular*}

\subsubsection{QCD parameters}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash as} & \as & \texttt{\textbackslash MSb} & \MSb & \texttt{\textbackslash lqcd} & \lqcd \\
\texttt{\textbackslash qsq} & \qsq &  \\
\end{tabular*}

\subsubsection{CKM, \boldmath \CP violation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eps} & \eps & \texttt{\textbackslash epsK} & \epsK & \texttt{\textbackslash epsB} & \epsB \\
\texttt{\textbackslash epsp} & \epsp & \texttt{\textbackslash CP} & \CP & \texttt{\textbackslash CPT} & \CPT \\
\texttt{\textbackslash T} & \T & \texttt{\textbackslash rhobar} & \rhobar & \texttt{\textbackslash etabar} & \etabar \\
\texttt{\textbackslash Vud} & \Vud & \texttt{\textbackslash Vcd} & \Vcd & \texttt{\textbackslash Vtd} & \Vtd \\
\texttt{\textbackslash Vus} & \Vus & \texttt{\textbackslash Vcs} & \Vcs & \texttt{\textbackslash Vts} & \Vts \\
\texttt{\textbackslash Vub} & \Vub & \texttt{\textbackslash Vcb} & \Vcb & \texttt{\textbackslash Vtb} & \Vtb \\
\texttt{\textbackslash Vuds} & \Vuds & \texttt{\textbackslash Vcds} & \Vcds & \texttt{\textbackslash Vtds} & \Vtds \\
\texttt{\textbackslash Vuss} & \Vuss & \texttt{\textbackslash Vcss} & \Vcss & \texttt{\textbackslash Vtss} & \Vtss \\
\texttt{\textbackslash Vubs} & \Vubs & \texttt{\textbackslash Vcbs} & \Vcbs & \texttt{\textbackslash Vtbs} & \Vtbs \\
\end{tabular*}

\subsubsection{Oscillations}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dm} & \dm & \texttt{\textbackslash dms} & \dms & \texttt{\textbackslash dmd} & \dmd \\
\texttt{\textbackslash DG} & \DG & \texttt{\textbackslash DGs} & \DGs & \texttt{\textbackslash DGd} & \DGd \\
\texttt{\textbackslash Gs} & \Gs & \texttt{\textbackslash Gd} & \Gd & \texttt{\textbackslash MBq} & \MBq \\
\texttt{\textbackslash DGq} & \DGq & \texttt{\textbackslash Gq} & \Gq & \texttt{\textbackslash dmq} & \dmq \\
\texttt{\textbackslash GL} & \GL & \texttt{\textbackslash GH} & \GH & \texttt{\textbackslash DGsGs} & \DGsGs \\
\texttt{\textbackslash Delm} & \Delm & \texttt{\textbackslash ACP} & \ACP & \texttt{\textbackslash Adir} & \Adir \\
\texttt{\textbackslash Amix} & \Amix & \texttt{\textbackslash ADelta} & \ADelta & \texttt{\textbackslash phid} & \phid \\
\texttt{\textbackslash sinphid} & \sinphid & \texttt{\textbackslash phis} & \phis & \texttt{\textbackslash betas} & \betas \\
\texttt{\textbackslash sbetas} & \sbetas & \texttt{\textbackslash stbetas} & \stbetas & \texttt{\textbackslash stphis} & \stphis \\
\texttt{\textbackslash sinphis} & \sinphis &  \\
\end{tabular*}

\subsubsection{Tagging}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash edet} & \edet & \texttt{\textbackslash erec} & \erec & \texttt{\textbackslash esel} & \esel \\
\texttt{\textbackslash etrg} & \etrg & \texttt{\textbackslash etot} & \etot & \texttt{\textbackslash mistag} & \mistag \\
\texttt{\textbackslash wcomb} & \wcomb & \texttt{\textbackslash etag} & \etag & \texttt{\textbackslash etagcomb} & \etagcomb \\
\texttt{\textbackslash effeff} & \effeff & \texttt{\textbackslash effeffcomb} & \effeffcomb & \texttt{\textbackslash efftag} & \efftag \\
\texttt{\textbackslash effD} & \effD & \texttt{\textbackslash etagprompt} & \etagprompt & \texttt{\textbackslash etagLL} & \etagLL \\
\end{tabular*}

\subsubsection{Key decay channels}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdToKstmm} & \BdToKstmm & \texttt{\textbackslash BdbToKstmm} & \BdbToKstmm & \texttt{\textbackslash BsToJPsiPhi} & \BsToJPsiPhi \\
\texttt{\textbackslash BdToJPsiKst} & \BdToJPsiKst & \texttt{\textbackslash BdbToJPsiKst} & \BdbToJPsiKst & \texttt{\textbackslash BsPhiGam} & \BsPhiGam \\
\texttt{\textbackslash BdKstGam} & \BdKstGam & \texttt{\textbackslash BTohh} & \BTohh & \texttt{\textbackslash BdTopipi} & \BdTopipi \\
\texttt{\textbackslash BdToKpi} & \BdToKpi & \texttt{\textbackslash BsToKK} & \BsToKK & \texttt{\textbackslash BsTopiK} & \BsTopiK \\
\texttt{\textbackslash Cpipi} & \Cpipi & \texttt{\textbackslash Spipi} & \Spipi & \texttt{\textbackslash CKK} & \CKK \\
\texttt{\textbackslash SKK} & \SKK & \texttt{\textbackslash ADGKK} & \ADGKK &  \\
\end{tabular*}

\subsubsection{Rare decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdKstee} & \BdKstee & \texttt{\textbackslash BdbKstee} & \BdbKstee & \texttt{\textbackslash bsll} & \bsll \\
\texttt{\textbackslash AFB} & \AFB & \texttt{\textbackslash FL} & \FL & \texttt{\textbackslash AT\#1 \textbackslash AT2} & \AT2 \\
\texttt{\textbackslash btosgam} & \btosgam & \texttt{\textbackslash btodgam} & \btodgam & \texttt{\textbackslash Bsmm} & \Bsmm \\
\texttt{\textbackslash Bdmm} & \Bdmm & \texttt{\textbackslash Bsee} & \Bsee & \texttt{\textbackslash Bdee} & \Bdee \\
\texttt{\textbackslash ctl} & \ctl & \texttt{\textbackslash ctk} & \ctk &  \\
\end{tabular*}

\subsubsection{Wilson coefficients and operators}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash C\#1 \textbackslash C9} & \C9 & \texttt{\textbackslash Cp\#1 \textbackslash Cp7} & \Cp7 & \texttt{\textbackslash Ceff\#1 \textbackslash Ceff9  } & \Ceff9   \\
\texttt{\textbackslash Cpeff\#1 \textbackslash Cpeff7} & \Cpeff7 & \texttt{\textbackslash Ope\#1 \textbackslash Ope2} & \Ope2 & \texttt{\textbackslash Opep\#1 \textbackslash Opep7} & \Opep7 \\
\end{tabular*}

\subsubsection{Charm}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash xprime} & \xprime & \texttt{\textbackslash yprime} & \yprime & \texttt{\textbackslash ycp} & \ycp \\
\texttt{\textbackslash agamma} & \agamma & \texttt{\textbackslash dkpicf} & \dkpicf &  \\
\end{tabular*}

\subsubsection{QM}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bra[1] \textbackslash bra\{a\}} & \bra{a} & \texttt{\textbackslash ket[1] \textbackslash ket\{b\}} & \ket{b} & \texttt{\textbackslash braket[2] \textbackslash braket\{a\}\{b\}} & \braket{a}{b} \\
\end{tabular*}

\subsection{Units (these macros add a small space in front)}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash unit[1] \textbackslash unit\{kg\}   } & \unit{kg}    &  \\
\end{tabular*}

\subsubsection{Energy and momentum }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tev} & \tev & \texttt{\textbackslash gev} & \gev & \texttt{\textbackslash mev} & \mev \\
\texttt{\textbackslash kev} & \kev & \texttt{\textbackslash ev} & \ev & \texttt{\textbackslash gevgev} & \gevgev \\
\texttt{\textbackslash mevc} & \mevc & \texttt{\textbackslash gevc} & \gevc & \texttt{\textbackslash mevcc} & \mevcc \\
\texttt{\textbackslash gevcc} & \gevcc & \texttt{\textbackslash gevgevcc} & \gevgevcc & \texttt{\textbackslash gevgevcccc} & \gevgevcccc \\
\end{tabular*}

\subsubsection{Distance and area (these macros add a small space)}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash km} & \km & \texttt{\textbackslash m} & \m & \texttt{\textbackslash ma} & \ma \\
\texttt{\textbackslash cm} & \cm & \texttt{\textbackslash cma} & \cma & \texttt{\textbackslash mm} & \mm \\
\texttt{\textbackslash mma} & \mma & \texttt{\textbackslash mum} & \mum & \texttt{\textbackslash muma} & \muma \\
\texttt{\textbackslash nm} & \nm & \texttt{\textbackslash fm} & \fm & \texttt{\textbackslash barn} & \barn \\
\texttt{\textbackslash mbarn} & \mbarn & \texttt{\textbackslash mub} & \mub & \texttt{\textbackslash nb} & \nb \\
\texttt{\textbackslash invnb} & \invnb & \texttt{\textbackslash pb} & \pb & \texttt{\textbackslash invpb} & \invpb \\
\texttt{\textbackslash fb} & \fb & \texttt{\textbackslash invfb} & \invfb & \texttt{\textbackslash ab} & \ab \\
\texttt{\textbackslash invab} & \invab &  \\
\end{tabular*}

\subsubsection{Time }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sec} & \sec & \texttt{\textbackslash ms} & \ms & \texttt{\textbackslash mus} & \mus \\
\texttt{\textbackslash ns} & \ns & \texttt{\textbackslash ps} & \ps & \texttt{\textbackslash fs} & \fs \\
\texttt{\textbackslash mhz} & \mhz & \texttt{\textbackslash khz} & \khz & \texttt{\textbackslash hz} & \hz \\
\texttt{\textbackslash invps} & \invps & \texttt{\textbackslash invns} & \invns & \texttt{\textbackslash yr} & \yr \\
\texttt{\textbackslash hr} & \hr &  \\
\end{tabular*}

\subsubsection{Temperature}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degc} & \degc & \texttt{\textbackslash degk} & \degk &  \\
\end{tabular*}

\subsubsection{Material lengths, radiation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Xrad} & \Xrad & \texttt{\textbackslash NIL} & \NIL & \texttt{\textbackslash mip} & \mip \\
\texttt{\textbackslash neutroneq} & \neutroneq & \texttt{\textbackslash neqcmcm} & \neqcmcm & \texttt{\textbackslash kRad} & \kRad \\
\texttt{\textbackslash MRad} & \MRad & \texttt{\textbackslash ci} & \ci & \texttt{\textbackslash mci} & \mci \\
\end{tabular*}

\subsubsection{Uncertainties}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sx} & \sx & \texttt{\textbackslash sy} & \sy & \texttt{\textbackslash sz} & \sz \\
\texttt{\textbackslash stat} & \stat & \texttt{\textbackslash syst} & \syst & \texttt{\textbackslash lumi} & \lumi \\
\end{tabular*}

\subsubsection{Maths}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash order} & \order & \texttt{\textbackslash chisq} & \chisq & \texttt{\textbackslash chisqndf} & \chisqndf \\
\texttt{\textbackslash chisqip} & \chisqip & \texttt{\textbackslash chisqvs} & \chisqvs & \texttt{\textbackslash chisqvtx} & \chisqvtx \\
\texttt{\textbackslash chisqvtxndf} & \chisqvtxndf & \texttt{\textbackslash deriv} & \deriv & \texttt{\textbackslash gsim} & \gsim \\
\texttt{\textbackslash lsim} & \lsim & \texttt{\textbackslash mean[1] \textbackslash mean\{x\}} & \mean{x} & \texttt{\textbackslash abs[1] \textbackslash abs\{x\}} & \abs{x} \\
\texttt{\textbackslash Real} & \Real & \texttt{\textbackslash Imag} & \Imag & \texttt{\textbackslash PDF} & \PDF \\
\texttt{\textbackslash sPlot} & \sPlot & \texttt{\textbackslash sFit} & \sFit &  \\
\end{tabular*}

\subsection{Kinematics}
\subsubsection{Energy, Momenta}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Ebeam} & \Ebeam & \texttt{\textbackslash sqs} & \sqs & \texttt{\textbackslash sqsnn} & \sqsnn \\
\texttt{\textbackslash pt} & \pt & \texttt{\textbackslash ptsq} & \ptsq & \texttt{\textbackslash ptot} & \ptot \\
\texttt{\textbackslash et} & \et & \texttt{\textbackslash mt} & \mt & \texttt{\textbackslash dpp} & \dpp \\
\texttt{\textbackslash msq} & \msq & \texttt{\textbackslash dedx} & \dedx &  \\
\end{tabular*}

\subsubsection{PID}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dllkpi} & \dllkpi & \texttt{\textbackslash dllppi} & \dllppi & \texttt{\textbackslash dllepi} & \dllepi \\
\texttt{\textbackslash dllmupi} & \dllmupi &  \\
\end{tabular*}

\subsubsection{Geometry}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degrees} & \degrees & \texttt{\textbackslash murad} & \murad & \texttt{\textbackslash mrad} & \mrad \\
\texttt{\textbackslash rad} & \rad &  \\
\end{tabular*}

\subsubsection{Accelerator}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash betastar} & \betastar & \texttt{\textbackslash lum} & \lum & \texttt{\textbackslash intlum[1] \textbackslash intlum\{2 \,\invfb\}} & \intlum{2 \,\invfb} \\
\end{tabular*}

\subsection{Software}
\subsubsection{Programs}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bcvegpy} & \bcvegpy & \texttt{\textbackslash boole} & \boole & \texttt{\textbackslash brunel} & \brunel \\
\texttt{\textbackslash davinci} & \davinci & \texttt{\textbackslash dirac} & \dirac & \texttt{\textbackslash evtgen} & \evtgen \\
\texttt{\textbackslash fewz} & \fewz & \texttt{\textbackslash fluka} & \fluka & \texttt{\textbackslash ganga} & \ganga \\
\texttt{\textbackslash gaudi} & \gaudi & \texttt{\textbackslash gauss} & \gauss & \texttt{\textbackslash geant} & \geant \\
\texttt{\textbackslash hepmc} & \hepmc & \texttt{\textbackslash herwig} & \herwig & \texttt{\textbackslash moore} & \moore \\
\texttt{\textbackslash neurobayes} & \neurobayes & \texttt{\textbackslash photos} & \photos & \texttt{\textbackslash powheg} & \powheg \\
\texttt{\textbackslash pythia} & \pythia & \texttt{\textbackslash resbos} & \resbos & \texttt{\textbackslash roofit} & \roofit \\
\texttt{\textbackslash root} & \root & \texttt{\textbackslash spice} & \spice & \texttt{\textbackslash urania} & \urania \\
\end{tabular*}

\subsubsection{Languages}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cpp} & \cpp & \texttt{\textbackslash ruby} & \ruby & \texttt{\textbackslash fortran} & \fortran \\
\texttt{\textbackslash svn} & \svn & \texttt{\textbackslash git} & \git & \texttt{\textbackslash latex} & \latex \\
\end{tabular*}

\subsubsection{Data processing}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash kbit} & \kbit & \texttt{\textbackslash kbps} & \kbps & \texttt{\textbackslash kbytes} & \kbytes \\
\texttt{\textbackslash kbyps} & \kbyps & \texttt{\textbackslash mbit} & \mbit & \texttt{\textbackslash mbps} & \mbps \\
\texttt{\textbackslash mbytes} & \mbytes & \texttt{\textbackslash mbyps} & \mbyps & \texttt{\textbackslash gbit} & \gbit \\
\texttt{\textbackslash gbps} & \gbps & \texttt{\textbackslash gbytes} & \gbytes & \texttt{\textbackslash gbyps} & \gbyps \\
\texttt{\textbackslash tbit} & \tbit & \texttt{\textbackslash tbps} & \tbps & \texttt{\textbackslash tbytes} & \tbytes \\
\texttt{\textbackslash tbyps} & \tbyps & \texttt{\textbackslash dst} & \dst &  \\
\end{tabular*}

\subsection{Detector related}
\subsubsection{Detector technologies}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash nonn} & \nonn & \texttt{\textbackslash ponn} & \ponn & \texttt{\textbackslash nonp} & \nonp \\
\texttt{\textbackslash cvd} & \cvd & \texttt{\textbackslash mwpc} & \mwpc & \texttt{\textbackslash gem} & \gem \\
\end{tabular*}

\subsubsection{Detector components, electronics}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tell1} & \tell1 & \texttt{\textbackslash ukl1} & \ukl1 & \texttt{\textbackslash beetle} & \beetle \\
\texttt{\textbackslash otis} & \otis & \texttt{\textbackslash croc} & \croc & \texttt{\textbackslash carioca} & \carioca \\
\texttt{\textbackslash dialog} & \dialog & \texttt{\textbackslash sync} & \sync & \texttt{\textbackslash cardiac} & \cardiac \\
\texttt{\textbackslash gol} & \gol & \texttt{\textbackslash vcsel} & \vcsel & \texttt{\textbackslash ttc} & \ttc \\
\texttt{\textbackslash ttcrx} & \ttcrx & \texttt{\textbackslash hpd} & \hpd & \texttt{\textbackslash pmt} & \pmt \\
\texttt{\textbackslash specs} & \specs & \texttt{\textbackslash elmb} & \elmb & \texttt{\textbackslash fpga} & \fpga \\
\texttt{\textbackslash plc} & \plc & \texttt{\textbackslash rasnik} & \rasnik & \texttt{\textbackslash elmb} & \elmb \\
\texttt{\textbackslash can} & \can & \texttt{\textbackslash lvds} & \lvds & \texttt{\textbackslash ntc} & \ntc \\
\texttt{\textbackslash adc} & \adc & \texttt{\textbackslash led} & \led & \texttt{\textbackslash ccd} & \ccd \\
\texttt{\textbackslash hv} & \hv & \texttt{\textbackslash lv} & \lv & \texttt{\textbackslash pvss} & \pvss \\
\texttt{\textbackslash cmos} & \cmos & \texttt{\textbackslash fifo} & \fifo & \texttt{\textbackslash ccpc} & \ccpc \\
\end{tabular*}

\subsubsection{Chemical symbols}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cfourften} & \cfourften & \texttt{\textbackslash cffour} & \cffour & \texttt{\textbackslash cotwo} & \cotwo \\
\texttt{\textbackslash csixffouteen} & \csixffouteen & \texttt{\textbackslash mgftwo} & \mgftwo & \texttt{\textbackslash siotwo} & \siotwo \\
\end{tabular*}

\subsection{Special Text }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eg} & \eg & \texttt{\textbackslash ie} & \ie & \texttt{\textbackslash etal} & \etal \\
\texttt{\textbackslash etc} & \etc & \texttt{\textbackslash cf} & \cf & \texttt{\textbackslash ffp} & \ffp \\
\texttt{\textbackslash vs} & \vs &  \\
\end{tabular*}

\subsubsection{Helpful to align numbers in tables}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash phz} & \phz &  \\
\end{tabular*}



==> wordcount.tex <==
\ProvidesFile{wordcount.tex}[2000/09/27 v1.5 Michael Downes]
% Copyright 2000 Michael John Downes
% This file has no restrictions on its use, distribution, or sale.
%
% If you run LaTeX on wordcount.tex it will prompt you for the name of a
% document to be counted. For most people, however, it will be more
% convenient to run the shell script wordcount.sh, giving the document
% name as the first argument. The comments in wordcount.sh
% give further information about the usage and limitations of this tool.

% The fundamental idea is to mark each character and interword space
% with a unique tag that will show up in TeX "showbox" output. Then
% arrange to make the output routine trigger a TeX overfull vbox message
% for the page box so that everything gets reported in the TeX log.
% Then run grep -c (or an equivalent text search utility, e.g., perl) on
% the log file to count the occurrences.
%
% In showbox output, a character is typically represented by a line of
% the form
%
%   ...\T1/cmr/m/n/10 e
%
% where "\T1/cmr/m/n/10" is the font name. We arrange things so that all
% characters are typeset in a font named "\3.08632". Furthermore, for
% interword spaces, which are normally represented in the output as
% something like
%
%   ...\glue 3.33333 plus 1.66666 minus 1.11111
%
% we use \spaceskip to ensure that it always appears as
%
%   ...\glue(\spaceskip) 3.08633 plus 9.0
%
% Then to count characters (including word spaces) we can
% grep for lines matching "3.0863", while to count words we
% count the number of lines in the log that match "3.08633" but not
% "3.08632".
%
% For an accurate count in multi-line paragraphs we also need
% to set rightskip to the flag value, since interword spaces are
% discarded at line breaks; and on the presumption that hyphenated
% compounds like "steady-state" should be counted as two words, we set
% \exhyphenpenalty to a value that ensures a line break at *every*
% explicit hyphen---then we will get a rightskip glue node between the
% two parts. (How about em-dashes? you may ask. Answer: it works all
% right, try it and see.)

\ifx\relax\?\def\wcQUIET{TT}\else\def\wcQUIET{TF}\fi

% We want accented letters to be represented by a single font char, to
% the extent possible:
\RequirePackage[T1]{fontenc}
\makeatletter
\thickmuskip=5.55555mu plus5.55555mu minus 2.22222mu
\let\@@thickmuskip\thickmuskip \newmuskip\thickmuskip
\let\@@spaceskip\spaceskip \xspaceskip=0pt
\newskip\@charfontname
% Ensure that these cannot be overridden.
\let\spaceskip\@charfontname \let\xspaceskip\spaceskip
\def\FreezeSpaces{%
  \setbox\z@\hbox{\mathsurround=\z@ $\mkern\@@thickmuskip$}%
  \@@spaceskip=\wd\z@ plus 9pt\relax
  % Setting rightskip to a slightly different value means that
  % end-of-line spaces can be distinguished if desired. (By default,
  % they are not.) Using fil units means there won't be any hyphenation
  % except for explicit hyphens.
  \dimen@\@@spaceskip \advance\dimen@ 1sp\relax
  \rightskip\z@ plus\strip@pt\dimen@ fil\relax
  % Prevent any further changes to \rightskip.
  \let\rightskip\spaceskip
  \@charfontname=\wd\z@ \advance\@charfontname -1sp\relax
  % Cancel all non-1000 sfcodes, which might otherwise affect the value
  % of inter-sentence spaces and keep them from being counted as
  % interword spaces.
  \def\do{\sfcode\fam\@m \advance\fam\@ne
    \ifnum\fam>\@cclv\expandafter\@gobble\fi \do
  }%
  \fam\z@ \do
  \let\frenchspacing\relax \let\nonfrenchspacing\relax
}
\def\DashPatch{%
  \exhyphenpenalty=-\@M \let\exhyphenpenalty\count@
  \hyphenpenalty\@M \let\hyphenpenalty\count@
  % LaTeX bug? Default definitions for these don't have \exhyphenpenalty
  % built in. Change them to just print a hyphen so that the penalties
  % will work.
  \def\textemdash{-}\def\textendash{-}%
}
% Here we set the font to ptmr8t (a T1 encoded font for which most
% people are likely to have a tfm file) and then make it difficult for
% the font to be changed ever again. We use two names for the font,
% \ptmr and \3.08632, the former being easier to use when resetting math
% fonts. The name that is defined last when TeX processes a document is
% the one that will be used in the log file.
\def\FreezeFont{%
  \expandafter\font
    \csname\strip@pt\@charfontname\endcsname
    =ptmr8t \relax
  \ptmr
  \check@mathfonts \let\check@mathfonts\relax
  \def\do{%
    \textfont\fam=\ptmr\scriptfont\fam=\ptmr\scriptscriptfont\fam=\ptmr
    \advance\fam\@ne \ifnum\fam<\sixt@@n \else\expandafter\@gobble\fi
    \do
  }%
  \fam=0 \do
}
\font\ptmr=ptmr8t \relax
\fontdimen22\ptmr=1sp % to permit use as math font 2
\let\selectfont\relax
\let\fontshape\@gobble \let\fontseries\@gobble \let\fontfamily\@gobble 
\let\fontencoding\@gobble \let\fontsize\@gobbletwo
\let\linespread\@gobble 
\let\try@load@fontshape\relax
\@namedef{U/msa/m/n}{}% disable special test in AMS documentclasses
\def\define@newfont{\expandafter\let\font@name=\ptmr}
\let\@@hfuzz\hfuzz \let\@@vfuzz\vfuzz
\newdimen\hfuzz \let\vfuzz\hfuzz
\def\QuietBoxes{%
  \@@hfuzz\maxdimen \@@vfuzz\maxdimen
}
\AtBeginDocument{\FreezeSpaces \FreezeFont \DashPatch \QuietBoxes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Halign patches
\def\ialign{\everycr{}\tabskip\@@spaceskip\halign} % initialized \halign
\def\extracolsep#1{\tabskip\@@spaceskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nofiles \let\makeindex\@empty % work-around for a natbib problem
% Seize control of the output routine to avoid extra clutter of dvi
% files. Handling \AtBeginDVI would take some extra work--for now I
% won't bother.
\def\showpagebox{%
  \showboxbreadth\maxdimen\showboxdepth99
  % This is a devious way of getting the box contents into the log file
  % without actually using \showbox (which typically results in a
  % nonzero exit code from the TeX run).
  \@@vfuzz\z@
  \setbox\z@\vbox to\z@{\box\@outputbox}%
  \setbox\z@\box\voidb@x
  \global \@colht \textheight
  \stepcounter{page}%
  \let\firstmark\botmark
}
\AtBeginDocument{\def\@outputpage{\showpagebox}}
\if\wcQUIET\else
\begingroup \def\msg^^J#1]^^J{\endgroup\message{#1]^^J^^J}}
\endlinechar=`\^^J \catcode`\ =12 \msg

The 'wordcount' utility provides a way of estimating the number of
words in a LaTeX document.

[Warning: The counting method uses a large log file as an intermediate
step. If your disk space is extremely low the counting process
may end prematurely for lack of space.]

\fi

% \typein has extraneous blank lines and slightly idiosyncratic prompt.
\begingroup \endlinechar=-1
\message{File name [press RETURN to cancel]: }
\def\do{%
  \let\do\@makeother \dospecials
  \global\read-1 to\wcFileName
  \endgroup
}
\do

\ifx\@empty\wcFileName
  \typeout{No file name given; quitting.}\expandafter\@@end\fi

\expandafter\filename@parse\expandafter{\wcFileName}
\edef\jobname{\filename@base}

\if\wcQUIET
  \message{\wcFileName}
\else
\typeout{^^JTo get a count of characters, run^^J^^J \space
%
  grep -c '3[.]0863[23]' wordcount.log^^J^^J%
%
or equivalent when processing is finished.^^J%
}
\fi

\typeout{Processing \wcFileName...^^J}

\IfFileExists{\wcFileName}{\batchmode}{\nonstopmode}
\edef\@tempa{\noexpand\makeatother
  \noexpand\input{\wcFileName}\noexpand\stop
}
\@tempa


==> words.tex <==
\clearpage

\section{Word count}
\label{sec:wors}

  
The paper has 2308 words, 4 figures (1127 words equivalent if we make Figs 2,3,4 two-column) and 1 equation (16 words equivalent), for a total of 3451 words.

\clearpage
